Digging Into Self-Supervised Learning of Feature Descriptors

Fully-supervised CNN-based approaches for learning local image descriptors have shown remarkable results in a wide range of geometric tasks. However, most of them require per-pixel ground-truth keypoint correspondence data which is difficult to acquire at scale. To address this challenge, recent weakly- and self-supervised methods can learn feature descriptors from relative camera poses or using only synthetic rigid transformations such as homographies. In this work, we focus on understanding the limitations of existing self-supervised approaches and propose a set of improvements that combined lead to powerful feature descriptors. We show that increasing the search space from in-pair to in-batch for hard negative mining brings consistent improvement. To enhance the discriminativeness of feature descriptors, we propose a coarse-to-fine method for mining local hard negatives from a wider search space by using global visual image descriptors. We demonstrate that a combination of synthetic homography transformation, color augmentation, and photorealistic image stylization produces useful representations that are viewpoint and illumination invariant. The feature descriptors learned by the proposed approach perform competitively and surpass their fully- and weakly-supervised counterparts on various geometric benchmarks such as image-based localization, sparse feature matching, and image retrieval.

==> hndesc_3dv2021_arXiv/assets/images/fig_pipeline.tex <==
\begin{figure*}[t!]
  \centering
    \includegraphics[width=\linewidth]{assets/images/raw/pipeline_small.pdf}
     \vspace{-15pt}
 \caption{\textbf{Overview of the proposed pipeline for learning local image descriptors.} Given an image and a set of interest points (top-left), we create a stylized copy of the image with a forward-pass through Style CNN. A pair of homography related crops ($c_i$) is randomly sampled from the original and stylized image in H-crops generator. We pass the image crops through Descriptor CNN to obtain representation of corresponding interest points in the feature space (embeddings). For each $a_i$ and $p_i$ descriptor from positive pair (anchors-positives), we create a list of hard-negative descriptors (shown with color gradient) using the proposed coarse-to-fine sampling procedure by leveraging global visual descriptors (Image retrieval block). Finally, the ranking loss %
 is utilized to optimize Descriptor CNN. See Sec.~\ref{sec:method} for a detailed description.}  
 \label{fig:pipeline_overview}
 \vspace{-5pt}
\end{figure*}

==> hndesc_3dv2021_arXiv/assets/images/fig_qualitative_matches.tex <==
\begin{figure*}[t!]
  \centering
    \includegraphics[width=1\linewidth]{assets/images/raw/quality_kpts_small.pdf}
 \caption{\textbf{Qualitative matching results.} We evaluate the proposed unsupervised pipeline with two different backbone models, R2D2 (top row) and CAPS (bottom row) on test samples of the MegaDepth dataset~\cite{Li2018Megadepth}. Both models have been trained on stylized images with color augmentations using in-batch hard negative sampling. Green lines indicate correspondences estimated by RANSAC (best viewed digitally). The proposed method predicts reliable matches even without training on annotated correspondences.}
 \label{fig:qualitative_results}
\end{figure*}

==> hndesc_3dv2021_arXiv/assets/plots/plt_mma.tex <==
\begin{figure*}[t!]
    \begin{minipage}{0.65\linewidth}
    \centering
    \includegraphics[width=\textwidth]{assets/plots/raw/hpatches_curves.pdf}
    \caption{\textbf{Mean matching accuracy (MMA) on the HPatches~\cite{Balntas2017HPatches} dataset.} For each method, the MMA with different pixel error thresholds is reported. The proposed self-supervised models (R2D2-U and CAPS-U) %
    achieve better overall performance for stricter matching thresholds (up to 3 pixels) compared to their supervised (R2D2-S and CAPS-S) counterparts. To avoid image clutter, for R2D2-U and CAPS-U, we only provide the results obtained by the {$\left(\squarehvfill,\squarerightblack\right)$} models.}
    \label{fig:hpatches_performance}
    \end{minipage}
    ~
    \begin{minipage}{0.34\linewidth}
        \centering
        \resizebox{\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{l | c c c | c c c }
		\toprule
		\multirowcell{2}{Method} & \multicolumn{3}{c|}{Illumination} & \multicolumn{3}{c}{Viewpoint} \\
		& \textEta & Precision & Recall & \textEta & Precision & Recall \\
		\midrule\midrule
		Root SIFT~\cite{Arandjelovic2012RootSIFT} & 0.933 & \textbf{0.782} & 0.799 & 0.566 & 0.651 & 0.527\\
		HardNet~\cite{Mishchuk2017HardNet} & 0.940 & 0.702 & 0.731 & 0.664 & 0.701 & 0.734\\
		SOSNet~\cite{Tian2019SOSNET} & 0.933 & 0.748 & 0.821 & \textbf{0.698} & 0.727 & 0.760\\
		SuperPoint~\cite{Detone18superpoint} & 0.912 & 0.710 & 0.811 & 0.671 & 0.685 & 0.750\\
		D2-Net~\cite{Dusmanu2019D2Net} & 0.905 & 0.725 & 0.775 & 0.617 & 0.666 & 0.664\\
		LISRD~\cite{Pautrat2020LISRD} & \textbf{0.947} & 0.766 & 0.920 & 0.688 & 0.731 & 0.757\\
		\textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & 0.940 & 0.762 & 0.837 & 0.692 & 0.720 & 0.732\\
		\textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & 0.888 & 0.757 & \textcolor{Cyan}{\underline{\textbf{0.938}}} & \textcolor{Cyan}{\underline{0.692}} & 0.723 & 0.699\\
		\midrule\midrule
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & 0.944 & 0.764 & \textcolor{Magenta}{\underline{0.838}} & 0.678 & \textcolor{Magenta}{\underline{0.732}} & \textcolor{Magenta}{\underline{0.739}} \\
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & 0.933 &	0.761 &	0.817 &	0.678 &	0.715 &	0.705  \\
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & \textcolor{Magenta}{\underline{\textbf{0.947}}} &	\textcolor{Magenta}{\underline{0.766}}	& 0.826 &	\textcolor{Magenta}{\underline{\textbf{0.698}}} &	0.726 &	0.720 \\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & 0.933 & 0.750 & 0.884 & 0.671 & 0.742 & 0.728 \\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & \textcolor{Cyan}{\underline{0.937}} &	0.756 &	0.893 &	0.661 &	0.740 &	0.752\\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & 0.919 & \textcolor{Cyan}{\underline{0.757}} & 0.890 & 0.681 & \textcolor{Cyan}{\underline{\textbf{0.747}}} & \textcolor{Cyan}{\underline{\textbf{0.762}}}\\
		\end{tabular}}
		\captionof{table}{\textbf{Evaluation results on HPatches.} We follow~\cite{Pautrat2020LISRD} and report the accuracy of homography estimation, precision and recall for error thresholds of 3 pixels. The best score between supervised baselines, \textcolor{Magenta}{R2D2} and \textcolor{Cyan}{CAPS}, and the proposed methods for each category is \underline{underlined}. The overall best score is in \textbf{bold}.}\label{tbl:hpatches_eval}
    \end{minipage}
    
\end{figure*}


==> hndesc_3dv2021_arXiv/assets/tables/ablation_all.tex <==
\begin{table}[t!]
    \begin{subtable}[t]{0.49\textwidth}
        \begin{center}
	    \resizebox{0.9\textwidth}{!}{%
		\footnotesize 		
		\begin{tabular}{c c c | c c }
		\toprule 
		\multirow{2}{*}{} & \multicolumn{2}{c|}{\multirowcell{2}{Metric}} & \multicolumn{2}{c}{Negative sampling type} \\
		& & & in-pair & in-batch \\ \midrule\midrule
		\multirow{4}{*}{\rotatebox[origin=c]{90}{$\cR$Oxford5k}} & \multirowcell{2}{mAP} & M & 55.38 & \textbf{58.69} \\
		& & H & 29.67 & \textbf{33.17} \\ \cmidrule{2-5}
		& \multirowcell{2}{mP@k $[1, 5, 10]$} & M & [94.29,	86.57, 78.43] & [\textbf{95.71}, \textbf{89.71}, \textbf{83.29}]\\
		& & H & [82.86, 54.57, 42.29] & [\textbf{85.71}, \textbf{60.29}, \textbf{45.71}]
        \\ \midrule\midrule
		\multirow{3}{*}{\rotatebox[origin=c]{90}{HPatches}} & \multirowcell{3}{MMA} & 1px & 0.239 / 0.425 / 0.332 & \textbf{0.254} / \textbf{0.439} / \textbf{0.346} \\
		& & 3px & 0.585 / 0.677 / 0.631 & \textbf{0.630} / \textbf{0.707} / \textbf{0.669} \\
		& & 5px & 0.648 / 0.742 / 0.695 & \textbf{0.706} / \textbf{0.784} / \textbf{0.745} \\[2pt] \midrule \midrule
		
		\multirow{2}{*}{\rotatebox[origin=c]{90}{Aachen}} &  & day & 87.9 / 94.2 / 97.9 &	\textbf{88.2} / \textbf{95.5} / \textbf{98.7} \\[1pt]
		& & night & 66.5 / 79.1 / 91.6 & \textbf{68.1} / \textbf{83.8} / \textbf{94.8} 
        \\[3pt] \midrule
        \end{tabular}
        }
	\end{center}
	\vspace{-15pt}
	\caption{\textbf{In-batch} \textit{vs.} \textbf{in-pair} hard negative sampling. Intra-batch negative mining performs consistently better over in-pair counterpart in all metrics. }\label{tbl:ablation_batch_vs_pair}
    \end{subtable}
        
    \begin{subtable}[h]{.49\textwidth}
        	\begin{center}
	\resizebox{0.9\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c c c | c | c c c }
		\toprule
		\multirow{2}{*}{} & \multicolumn{2}{c|}{\multirowcell{2}{Metric}} & \multirowcell{2}{Baseline} & \multicolumn{3}{c}{Negative samples in mini-batch} \\
		& & & & $all$ & $random$ & $top$-$k$ \\ \midrule\midrule
		\multirow{12}{*}{\rotatebox[origin=c]{90}{$\cR$Oxford5k}} & \multirowcell{3}{mAP} & E & $72.60$ & \underline{72.85} & $72.06$ & $\textbf{75.27}$ \\
		& & M & $54.89$ & \underline{57.06} & $56.91$ & $\textbf{57.83}$ \\
		& & H & $27.37$ & \underline{30.53} & $31.28$ & $\textbf{31.56}$ \\ \cmidrule{2-7}
		& \multirowcell{9}{mP@k $[1, 5, 10]$} & \multirowcell{3}{E} & $94.12$	& $\textbf{97.06}$ &	\underline{95.59} & $\textbf{97.06}$ \\
		& & & $80.74$ & $84.41$ & \underline{84.63} & $\textbf{88.24}$ \\
		& & & $74.12$ & $77.40$ & \underline{77.72} & $\textbf{80.44}$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{M} & $91.43$ & $\textbf{95.71}$ & $94.29$ & $\textbf{95.71}$ \\
		& & & $80.57$ & \underline{88.10} & $\textbf{88.86}$ & $\textbf{88.86}$ \\
		& & & $73.86$ & \underline{81.24} & $81.00$ & $\textbf{81.41}$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{H} & $61.43$ & \underline{81.43} & \underline{81.43} & $\textbf{82.86}$ \\
		& & & $47.50$ & $56.43$ & \underline{57.14} & $\textbf{59.43}$ \\
		& & & $39.79$ & $43.57$ & \underline{44.57} & $\textbf{45.43}$ \\ \midrule\midrule
		\multirowcell{3}{\rotatebox[origin=c]{90}{ Tokyo24/7}} & \multirowcell{3}{recall} & r@1 & $67.10$ & \underline{76.15} & $74.92$ & $\textbf{79.05}$ \\[2pt]
		& & r@5 & $74.20$ & \underline{81.27} & $80.63$ & $\textbf{84.13}$ \\[2pt]
		& & r@10 & $76.10$ & \underline{83.49} & $81.90$ & $\textbf{85.71}$ \\[2pt] \midrule
		\multirow{6}{*}{\rotatebox[origin=c]{90}{Aachen v1.1}} & \multirowcell{6}{$0.25m, 2^\circ$ \\ $0.5m, 5^\circ$ \\ $5m, 10^\circ$} & \multirowcell{3}{day} & \underline{87.7} & $87.5$ & $88.0$ & $\textbf{88.0}$ \\
		& & & \underline{94.7} & $94.4$ & 94.2 & $\textbf{94.8}$ \\
		& & & \textbf{98.7} & \underline{98.3} & $98.1$ & $98.2$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{night} & \underline{69.6} & $\textbf{70.2}$ & $67.0$ & $\textbf{70.2}$ \\
		& & & \textbf{86.4} & \underline{85.9} & 84.3 & \textbf{86.4} \\
		& & & \underline{95.3} & \textbf{95.8} & $94.8$ & \textbf{95.8} \\ \midrule
		\multirow{6}{*}{\rotatebox[origin=c]{90}{InLoc}} & \multirowcell{6}{$0.25m, 2^\circ$ \\ $0.5m, 5^\circ$ \\ $5m, 10^\circ$} & \multirowcell{3}{DUC1} & \underline{27.8} & \textbf{28.3} & 27.3 & \underline{27.8}  \\
		& & & 42.4 & \textbf{46.0} & 43.4 & \underline{43.9} \\
		& & & \underline{54.4} & \textbf{55.6} & 53.0 & 54.0 \\ \cmidrule{3-7}
		& & \multirowcell{3}{DUC2} & 22.1 & 23.7 & \underline{26.0} & \textbf{27.5} \\
		& & & 34.4 & 35.1 & \underline{36.6} & \textbf{38.2} \\
		& & & 42.7 & 40.5 & \underline{44.3} & \textbf{49.6} \\ \midrule
		\end{tabular}
		
	}
	
	\end{center}
	\vspace{-15pt}
	\caption{\textbf{Intra-batch negative sampling}. For a listwise loss, the $top$-$k$ sampling strategy leads to a better performance over its counterparts in almost all metrics. The best score is in bold and the second best score is underlined.}\label{tbl:ablation_topK_vs_all}
    \end{subtable}
    \vspace{-5pt}
    \caption{\textbf{Ablation study.} We analyze the influence of different design choices of the proposed approach. See Sec.~\ref{sec:ablation} for more details.}
    \vspace{-15pt}
\end{table}


==> hndesc_3dv2021_arXiv/assets/tables/res_localization_all.tex <==
\begin{table*}[t!]
    \begin{subtable}[h]{0.7\textwidth}
        \begin{center}
	    \resizebox{\textwidth}{!}{%
		\footnotesize 		
		\begin{tabular}{c l | c c | c c c | c c c | c c c | c c c}
		\toprule
		\multirow{4}{*}{} & \multirowcell{4}{Method} & \multirowcell{4}{Supervision} & \multirowcell{4}{Training\\data} & \multicolumn{6}{c}{Aachen v1.1} & \multicolumn{6}{|c}{InLoc} \\
		& & & & \multicolumn{6}{c}{\% localized queries} & \multicolumn{6}{|c}{\% localized queries} \\
		& & & & \multicolumn{3}{c|}{Day (824 images)} & \multicolumn{3}{c}{Night (191 images)} & \multicolumn{3}{|c|}{DUC1} &  \multicolumn{3}{c}{DUC2} \\
		& & & & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ \\ \midrule\midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Super}} & \textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & OF & A+R & \textcolor{Magenta}{\textbf{88.6}} & \textcolor{Magenta}{\textbf{95.4}} & \textcolor{Magenta}{\textbf{98.9}} & 72.8 & 89.0 & 97.4 & 27.8 & 42.4 & 54.5 & 22.1 & 34.4 & 42.7 \\
        & \textcolor{Magenta}{R2D2*} & OF & A & 87.7 & 94.7 & 98.7 & 69.6 & 86.4 & 95.3 & 29.8 & 43.4 & 55.1 & 21.4 & 34.4 & 43.5 \\
        & \textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & SL+RP & M & 85.3 & \textcolor{Cyan}{\textbf{93.8}} & 97.9 & \textcolor{Cyan}{\textbf{75.9}} & 88.5 & \textcolor{Cyan}{\textbf{97.9}} & 38.4 & 59.1 & \textcolor{Cyan}{\textbf{74.7}} & 34.4 & 52.7 & 61.8\\ \midrule\midrule
        \multirow{11}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-$\left(\squarehvfill\right)$ & - & A & 87.4 & 94.9 & 98.3 & 63.9 & 80.1 & 92.1 & \textcolor{Magenta}{\textbf{29.3}} & 46.5 & 57.6 & 29.8 & 42.0 & 51.1 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & A & 88.0 & 94.8 & 98.2 & 70.2 & 86.4 & 95.8 & 27.8 & 46.5 & 57.6 & 29.8 & 42.0 & 51.1\\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M & 87.4 & 94.7 & 98.3 & 72.3 & 88.5 & 97.4 & 26.8 & 46.0 & 57.1 & 26.7 & \textcolor{Magenta}{\textbf{42.7}} & 48.9 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & - & M & 87.5 & 94.9 & 98.3 & 71.7 & 86.4 & 96.9 & 27.8 & 43.4 & 54.5 & 28.2 & 41.2 & 51.9 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & - & M & 88.1 & 94.8 & 98.1 & 71.2 & 88.0 & 95.8 & 30.8 & 43.9 & 54.0 & 28.2 & 37.4 & 46.6\\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M+P & 88.2 & 95.1 & 98.5 & \textcolor{Magenta}{\textbf{73.3}} & \textcolor{Magenta}{\textbf{90.1}} & \textcolor{Magenta}{\textbf{97.4}} & \textcolor{Magenta}{\textbf{29.3}} & \textcolor{Magenta}{\textbf{47.0}} & \textcolor{Magenta}{\textbf{58.1}} & \textcolor{Magenta}{\textbf{25.2}} & 41.2 & \textcolor{Magenta}{\textbf{51.9}} \\ 
        \cmidrule{2-16}
        & CAPS-{$\left(\squarehvfill\right)$} & - & M & 85.8 & 93.8 & 98.2 & 67.0 & 82.2 & 96.9 &35.9 & 54.0 & 69.2 & 38.9 & 50.4 & 64.9\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M & 85.1 & 93.2 & 97.8 & 71.7 & 87.4 & \textcolor{Cyan}{\textbf{97.9}} & \textcolor{Cyan}{\textbf{39.9}} & \textcolor{Cyan}{\textbf{61.6}} & 70.7 & 38.2 & 51.1 & \textcolor{Cyan}{\textbf{66.4}}\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & - & M & \textcolor{Cyan}{\textbf{87.0}} & \textcolor{Cyan}{\textbf{93.8}} & \textcolor{Cyan}{\textbf{98.3}} & 73.8 & \textcolor{Cyan}{\textbf{89.0}} & 97.4 & 35.9 & 53.0 & 65.7 & 32.8 & 47.3 & 61.1\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & - & M & 86.9 & \textcolor{Cyan}{\textbf{93.8}} & 98.1 & 71.7 & \textcolor{Cyan}{\textbf{89.0}} & 97.4 & 35.9 & 53.5 & 64.6 & 30.5 & 45.0 & 58.8 \\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M+P & 85.4 & 93.2 & 97.9 & 72.3 & 88.5 & \textcolor{Cyan}{\textbf{97.9}} & 38.9 & 56.1 & 69.2 & \textcolor{Cyan}{\textbf{40.5}} & \textcolor{Cyan}{\textbf{54.2}} & \textcolor{Cyan}{\textbf{66.4}}\\
		\end{tabular}
        }
	\end{center}
	\vspace{-5pt}
	\caption{Evaluations results for Aachen v1.1~\cite{Zhang2020AachenV11} and InLoc~\cite{Taira2018InLoc} }\label{tbl:loc_aachen_inloc}
    \end{subtable}
    ~
    \begin{subtable}[h]{.29\textwidth}
        	\begin{center}
	\resizebox{.9\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c l|l l l}
        \multirow{2}{*}{} & \multirow{2}{*}{Method} & \multicolumn{3}{|c}{Recall} \\
        & & \multicolumn{1}{|c}{r@1} & \multicolumn{1}{c}{r@5} & \multicolumn{1}{c}{r@10}\\
    \hline
    \hline
    & DenseVLAD~\cite{Torii2015Tokyo247} & 67.10 & 74.20 & 76.10 \\
    & NetVLAD-TokyoTM~\cite{Arandjelovic2016NetVLAD} & 71.10 & 83.10 & 86.20 \\
    & SIFT~\cite{Lowe2004SIFT} & 73.33 & 80.00 & 84.40 \\
    & InLoc~\cite{Taira2018InLoc} & 62.54 & 67.62  & 70.48 \\
    & Dense Pixel Matching~\cite{Laskar2020DensePixelMatching} & 77.14 & 84.44 & 86.67 \\
    & \textcolor{Magenta}{R2D2}-[A+R]~\cite{Revaud2019R2D2} & 78.10 & 82.54 & 84.13 \\
    & \textcolor{Cyan}{CAPS}-[M]~\cite{Wang2020CAPS} & \textcolor{Cyan}{\textbf{83.49}} & 86.67 & 87.94 \\ \hline \hline
    \multirow{9}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[A] & 79.05 & 83.17 & 85.71 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[M] & 79.37 & \textcolor{Magenta}{\textbf{84.76}} & 85.71 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd-[M] & 78.41 & 82.54 & 83.81 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd-[M] & 77.78 & 82.86 & 85.40 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[M+P] & \textcolor{Magenta}{\textbf{79.68}} & 84.44 & \textcolor{Magenta}{\textbf{86.03}} \\ \cmidrule{2-5}
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-[M] & 82.54 & 86.03 & 87.94 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd-[M] & 81.27 & 85.71 & 86.98 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd-[M] & 82.54 & 86.35 & 87.94 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-[M+P] & 82.86 & \textcolor{Cyan}{\textbf{87.30}} & \textcolor{Cyan}{\textbf{88.25}} \\

    \end{tabular}
		
	}
	
	\end{center}
	\vspace{-10pt}
	\caption{Performance on Tokyo24/7~\cite{Torii2015Tokyo247}}\label{tbl:loc_tokyo247}
    \end{subtable}
    
    \vspace{-5pt}
    \caption{\textbf{Indoor and outdoor localization performance}. The supervised baseline methods, \textcolor{Magenta}{R2D2} and \textcolor{Cyan}{CAPS}, are color-coded. Best results in each category for each localization benchmark are in \textbf{bold}. \textbf{Legend}: \textit{Supervision}: OF~--~ground-truth pixel correspondences based on optical flow~\cite{Revaud2019R2D2}; SL~--~ground-truth scene labels; RP~--~relative camera poses. \textit{Training data}: A~--~Aachen database images; R~--~Random images from the Internet~\cite{Revaud2019R2D2}; M~--~MegaDepth dataset; P~--~Phototourism dataset. For Tokyo24/7, the training datasets for our supervised baselines and the proposed approach are given in $\left[.\right]$ parentheses.}
    
\end{table*}


==> hndesc_3dv2021_arXiv/assets/tables/res_retrieval.tex <==
\begin{table*}[t!]
	\begin{center}
	\resizebox{.99\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c l | c c | c c c | c c c | c c c | c c c | c c c |  c c c | c c c | c c c}
		\toprule
		 \multirow{3}{*}{} & \multirowcell{3}{Method} & \multirowcell{3}{Training\\data} & \multirowcell{3}{Hard-negative\\mining} & \multicolumn{12}{|c}{$\cR$Oxford5k} & \multicolumn{12}{|c}{$\cR$Paris6k} \\
	     & & & & \multicolumn{3}{c}{mAP} & \multicolumn{9}{|c|}{mP@k [1, 5, 10]} & \multicolumn{3}{c}{mAP} & \multicolumn{9}{|c}{mP@k [1, 5, 10]} \\
		 & & & & E & M & H & \multicolumn{3}{c|}{E} & \multicolumn{3}{c|}{M} & \multicolumn{3}{c|}{H} & E & M & H & \multicolumn{3}{c|}{E} & \multicolumn{3}{|c|}{M} &  \multicolumn{3}{c}{H} \\ \midrule\midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{Supervised}} & Baseline~\cite{Radenovic2016GEM} & - & - & 72.60 & 54.89 &	27.37 & 91.43 & 80.74 & 74.12 & 91.43 & 80.57 & 73.86 & 61.43 & 47.50 & 39.79 & 86.15 & 68.98 & 43.86 & 98.57 & 95.14 & 93.43 & 98.57 & 98.57 & 96.14 & 95.71 & 87.71 & 82.86\\
		& \textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & A+R & in-pair & 76.39 & \textcolor{Magenta}{\textbf{59.09}} & \textcolor{Magenta}{\textbf{33.20}} & 97.06 & 88.38 & 81.55 & 95.71 & 89.71 & 83.57 & \textcolor{Magenta}{\textbf{85.71}} & \textcolor{Magenta}{\textbf{61.14}} & \textcolor{Magenta}{\textbf{47.14}} & 85.73 & 68.51 & 42.86 & \textcolor{Magenta}{\textbf{100}} & 97.24 & 95.81 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{100}} & 99.14 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{92.57}} & 81.57\\
		& R2D2* & A & in-pair & 75.36 & 58.61 & 32.69 & 97.06 & 87.35 & 79.56 & 95.71 & 89.43 & 82.57 & 85.71 & 59.14 & 45.86 & 85.39 & 68.36 & 42.93 & 100 & 97.43 & 96.14 & 100 & 99.71 & 98.86 & 98.57 & 91.14 & 82.43\\
        & \textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & M & - & 75.27 & 59.67 & \textcolor{Cyan}{\textbf{34.77}} & 94.12 & 86.76 & 80.44 & 94.29 & 89.14 & 84.14 & \textcolor{Cyan}{\textbf{85.71}} & \textcolor{Cyan}{\textbf{66.00}} & \textcolor{Cyan}{\textbf{50.57}} & \textcolor{Cyan}{\textbf{88.92}} & \textcolor{Cyan}{\textbf{69.87}} & \textcolor{Cyan}{\textbf{44.47}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{99.43}} & \textcolor{Cyan}{\textbf{97.43}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 98.57 & \textcolor{Cyan}{\textbf{94.86}} & \textcolor{Cyan}{\textbf{87.14}}\\ \midrule\midrule
		& R2D2-$\left(\squarehvfill\right)$ & M & in-pair & 70.99 & 55.38 & 29.67 & 95.59 & 84.12 & 75.44 & 94.29 & 86.57 & 78.43 & 82.86 & 54.57 & 42.29 & 84.57 & 67.95 & 42.57 & 100 & 97.14 & 96.00 & 100 & 100 & 99.14 & 100 & 90.29 & 81.86  \\
        \multirow{8}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-$\left(\squarehvfill\right)$ & A & in-batch & 73.16 & 56.47 & 30.05 & 95.59 & 85.51 & 77.87 & 94.29 & 87.14 & 79.29 & 82.86 & 55.43 & 42.57 & 86.09 & 68.60 & \textcolor{Magenta}{\textbf{43.04}} & 100 & 98.00 & 96.43 & 100 & 99.71 & 99.43 & 97.14 & 91.71 & \textcolor{Magenta}{\textbf{82.71}}  \\
		& R2D2-$\left(\squarehvfill\right)$ & M & in-batch & 75.09 & 58.69 & 33.17 & 97.06 & 87.06 & 80.15 & 95.71 & 89.71 & 83.29 & 85.71 & 60.29 & 45.71 & 86.38 & 68.60 & 42.83 & 100 & 98.00 & \textcolor{Magenta}{\textbf{96.86}} & 100 & 100 & \textcolor{Magenta}{\textbf{99.57}} & 98.57 & 91.43 & 82.57 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & M & in-batch & 75.70 & 58.79 & 33.03 & 97.06 & 86.57 & 80.88 & 95.71 & 89.14 & 82.57 & 88.57 & 60.00 & 46.29 & 86.49 & 68.67 & 42.86 & 100 & 98.29 & 96.43 & 100 & 100 & 99.29 & \textcolor{Magenta}{\textbf{100}} & 92.00 & 82.14 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & M & in-batch & 75.97 & 58.70 & 32.85 & 97.06 & 88.24 & 81.03 & 95.71 & \textcolor{Magenta}{\textbf{90.00}} & 83.14 & 85.71 & 60.29 & 46.86 & 86.31 & 68.63 & 42.85 & 100 & 98.00 & 96.29 & 100 & 100 & 99.43 & 100 & 91.14 & \textcolor{Magenta}{\textbf{82.71}} \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & M & in-batch & 73.47 & 57.57 & 32.16 & 97.06 & 85.59 & 76.91 & 95.71 & 88.86 & 81.29 & 85.71 & 58.57 & 46.43 & 86.04 & 68.48 & 42.76 & 100 & 97.71 & 96.14 & 100 & 99.71 & 99.29 & 98.57 & 89.71 & 82.29 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & M+P & in-batch & \textcolor{Magenta}{\textbf{76.65}} & 59.07 & 33.15 & \textcolor{Magenta}{\textbf{97.06}} & \textcolor{Magenta}{\textbf{88.82}} & \textcolor{Magenta}{\textbf{81.62}} & \textcolor{Magenta}{\textbf{95.71}} & 89.43 & \textcolor{Magenta}{\textbf{83.71}} & \textcolor{Magenta}{\textbf{85.71}} & 60.57 & \textcolor{Magenta}{\textbf{47.14}} & \textcolor{Magenta}{\textbf{87.02}} & \textcolor{Magenta}{\textbf{68.80}} & 42.85 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{98.57}} & \textcolor{Magenta}{\textbf{96.86}} & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{99.57}} & 98.57 & 91.43 & 81.86 \\ \cmidrule{2-28}
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & M & in-batch & 74.68 & 58.64 & 32.54 & 95.59 & 87.06 & 78.38 & 94.29 & 89.71 & 82.71 & 82.86 & 59.14 & 46.29 & 87.88 & 69.25 & 43.46 & 100 & 99.14 & 96.71 & 100 & 100 & 99.71 & 100 & 92.86 & 84.14 \\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & M & in-batch & 77.06 & 59.67 & 32.89 & 95.59 & 88.82 & \textcolor{Cyan}{\textbf{82.04}} & 94.29 & 90.57 & \textcolor{Cyan}{\textbf{84.71}} & 82.86 & 60.00 & 47.57 & 87.36 & 69.19 & 43.54 & 100 & 98.86 & 96.71 &  100 & 100 & 99.86 & 100 & 94.00 & 84.71 \\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & M & in-batch & \textcolor{Cyan}{\textbf{77.17}} & 59.54 & 32.71 & \textcolor{Cyan}{\textbf{97.06}} & \textcolor{Cyan}{\textbf{89.85}} & 81.47 & \textcolor{Cyan}{\textbf{95.71}} & \textcolor{Cyan}{\textbf{90.86}} & 84.43 & \textcolor{Cyan}{\textbf{85.71}} & 60.57 & 47.29 & 87.61 & 69.14 & 43.33 & \textcolor{Cyan}{\textbf{100}} & 98.86 & 96.71 & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 99.57 & \textcolor{Cyan}{\textbf{100}} & 93.43 & 83.71\\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & M+P & in-batch & 76.49 & \textcolor{Cyan}{\textbf{59.72}} & 33.60 & 95.59 & 88.16 & 81.54 & 94.29 & 89.71 & 84.14 & 84.29 & 62.00 & 48.14 & 87.66 & 69.12 & 43.34 & \textcolor{Cyan}{\textbf{100}} & 98.86 & 97.00 & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 100 & 100 & 93.14 & 84.71\\
		\end{tabular}
	}
	\caption{\textbf{Image retrieval performance}. We report results for the $\cR$Oxford5k and $\cR$Paris6k datasets following the evaluation protocol proposed in~\cite{Radenovic2018Revisited}. We use the same color-map for the supervised baseline approaches as in Table~\ref{tbl:loc_aachen_inloc}. The proposed unsupervised models demonstrate competitive performance 
	\vspace{-5mm}
	\label{tbl:image_retrieval_results}}
	\end{center}

\end{table*}


==> hndesc_3dv2021_arXiv/sections/ablation.tex <==
\section{Ablation Study}\label{sec:ablation}
The goal of this section is to investigate the benefits of using intra-batch hard negative mining compared to in-pair sampling used in recent CNN-based interest point detectors and descriptors~\cite{Dusmanu2019D2Net,Revaud2019R2D2}. For in-batch negative mining, we experiment with different sampling strategies: consider \textit{all} negative samples in a mini-batch, take $k$ negative samples \textit{randomly}, and consider only $top$-$k$ samples.

\customparagraph{In-pair \textit{vs.} in-batch negative mining.} To evaluate the effectiveness of the sampling procedure we conduct controlled experiments summarized in Table~\ref{tbl:ablation_batch_vs_pair}. The results are obtained by the R2D2-{$\left(\squarehvfill\right)$} model trained on the MegaDepth dataset using the AP loss function. We use the following evaluation benchmarks: sparse feature matching (HPatches), image retrieval ($\cR$Oxford5k), and visual localization (Aachen v1.1) (see Sec.~\ref{ssec:benchmarks_metrics}). As shown in Table~\ref{tbl:ablation_batch_vs_pair}, in-batch hard-negative sampling significantly outperforms in-pair mining in all metrics. We observe similar behaviour with metric learning losses, \eg, Triplet loss. The results obtained by models trained with Triplet loss are provided in supplementary.

\customparagraph{In-batch sampling: all \textit{vs.} random \textit{vs.} topK.} In contrast to \textit{pairwise} ranking losses, the AP loss is defined on a ranked list of samples $L$. Let us assume we have a mini-batch consisting of $M$ homography related image crop pairs where each crop has $p$ interest points extracted by SuperPoint~\cite{Detone18superpoint} detector. Each keypoint is associated with a feature vector and has one positive and $M\times(p-1)$ negative samples within a mini-batch. Therefore, we consider 3 ways of constructing the list $L$: take all possible negatives, randomly select $k$ samples from $M\times(p-1)$, and select $top$-$k$ negatives (the proposed strategy). For each setting, we train our unsupervised R2D2-{$\left(\squarehvfill\right)$} model on (A) and evaluate on two benchmarks: image retrieval and image-based localization. The results are presented in Table~\ref{tbl:ablation_topK_vs_all}. The proposed "top-k negative" sampling approach surpasses its counterparts with a noticeable margin. The number of hard negative samples $k$ is set to 30 after empirical evaluation for all our experiments. Interestingly, unlike Triplet loss~\cite{Mishchuk2017HardNet}, the AP loss with random sampling will \textit{not} lead to overfit, but evaluation performance is low.


\input{assets/tables/ablation_all}

==> hndesc_3dv2021_arXiv/sections/abstract.tex <==
Fully-supervised CNN-based approaches for learning local image descriptors have shown remarkable results in a wide range of geometric tasks. However, most of them require per-pixel ground-truth keypoint correspondence data which is difficult to acquire at scale. To address this challenge, recent weakly- and self-supervised methods can learn feature descriptors from relative camera poses or using only synthetic rigid transformations such as homographies. In this work, we focus on understanding the limitations of existing self-supervised approaches and propose a set of improvements that combined lead to powerful feature descriptors. We show that increasing the search space from in-pair to in-batch for hard negative mining brings consistent improvement. To enhance the discriminativeness of feature descriptors, we propose a coarse-to-fine method for mining local hard negatives from a wider search space by using global visual image descriptors. We demonstrate that a combination of synthetic homography transformation, color augmentation, and photorealistic image stylization produces useful representations that are viewpoint and illumination invariant. The feature descriptors learned by the proposed approach perform competitively and surpass their fully- and weakly-supervised counterparts on various geometric benchmarks such as image-based localization, sparse feature matching, and image retrieval. 








==> hndesc_3dv2021_arXiv/sections/conclusion.tex <==
\section{Conclusion}
In this work, we have presented a self-supervised local descriptor learning framework. We introduced three main contributions: (1) a coarse-to-fine method to efficiently sample hard-negative local descriptors by leveraging visual image descriptors, (2) the modified version of AP loss which can carefully handle imbalance between the number of positive and negative keypoint descriptors and (3) photorealistic image stylization that combined with synthetic color augmentation can significantly enhance the robustness of learned local descriptors to illumination changes. The proposed improvements together result in a self-supervised approach demonstrates favourable performance on a wide range of geometric tasks compared to strong fully- and weakly-supervised baseline models.



==> hndesc_3dv2021_arXiv/sections/experiments.tex <==
\section{Experiments} \label{sec:experiments_results}
Here, we describe the experimental setting and validate that (1) increasing the search space from within-pair to intra-batch for hard negative mining improves the discriminativeness of local image descriptors and leads to better performance, (2) photorealistic image stylization in addition to color augmentations demonstrates good generalization performance and improves results, especially when query images are taken during challenging illumination conditions, (3) self-supervised methods for local image descriptors learning achieve competitive results with their fully- and weakly-supervised counterparts. In order to highlight the effectiveness of the proposed ideas, we further present an extensive ablation study.

\input{assets/plots/plt_mma}

\subsection{Baselines}\label{ssec:baselines}
In this work, we consider two recent approaches, R2D2~\cite{Revaud2019R2D2} and CAPS~\cite{Wang2020CAPS}, as the baseline methods. Since we focus exclusively on local image descriptors learning, SuperPoint~\cite{Detone18superpoint} keypoint detector is used in all our experiments and the baselines.

\customparagraph{R2D2}~\cite{Revaud2019R2D2} can directly extract dense descriptors and a heatmap of keypoints from an input image. It consists of L2-Net backbone network with two heads for jointly learning repeatable and reliable matches. The network was trained on pairs of image crops with known pixel correspondences based on either synthetic homography or 3D reprojection. We consider the model trained with 3D supervision as our baseline.

\customparagraph{CAPS}~\cite{Wang2020CAPS} is a CNN-based local image descriptor trained in a weakly-supervised manner. Specifically, it can learn feature descriptors using only scene labels and relative camera poses between views. It utilizes SuperPoint keypoints and an epipolar constraint on pixel locations of matched points as a supervision signal. The resulting descriptor consists of two concatenated 128-dimensional feature vectors, \ie coarse- and fine-level descriptors, extracted at different parts of the model encoder (an ImageNet-pretrained ResNet-50 architecture~\cite{Deng2009ImageNet,He2016ResNet}). In our experiments, we utilize \textit{only} fine-level descriptors to optimize the proposed criterion (Eq.~\ref{eq:ap_loss}).



\input{assets/images/fig_qualitative_matches}

\input{assets/tables/res_localization_all}

\subsection{Notations}\label{ssec:notations}
We use the following symbolic notation throughout the paper: {$\left(\squarehvfill\right)$} denotes models trained with synthetic CA; {$\left(\squarerightblack\right)$} indicates photorealistic stylized images; {$\left(\squarehvfill,\squarerightblack\right)$} if both CA and style transfer are used during training. Finally, we refer the models utilizing image retrieval pre-trained networks for extracting visual descriptors with a suffix~\texttt{*-gd} and~\texttt{*-selfgd} denotes the self-supervised way of computing visual descriptors on the fly using the current state of the proposed Descriptor CNN (\cf Figure~\ref{fig:pipeline_overview}).


\subsection{Benchmarks and metrics}\label{ssec:benchmarks_metrics}
We verify the proposed ideas on the following benchmarks.

\customparagraph{Sparse feature matching.} For this experiment, we evaluate our descriptors on the full images provided by the HPatches dataset~\cite{Balntas2017HPatches}. The dataset consists of 116 image sequences with varying photometric and viewpoint changes. Each sequence contains a reference image and 5 source images taken under a different viewpoint. For all image pairs, the estimated ground-truth homography matrix with respect to the reference image is provided. We follow the standard evaluation protocol~\cite{Dusmanu2019D2Net} and use the mean matching accuracy (MMA) as the metric, \ie the average percentage of correct matches per image under a certain pixel threshold. In addition to MMA, we also report a homography estimation score~\cite{Detone18superpoint,Dusmanu2019D2Net}, precision and recall computed for a 3-pixel error threshold. %

\customparagraph{Image-based localization.} To verify the generalization performance of the proposed approach, we evaluate our method on indoor and outdoor visual localization benchmarks. Specifically, we consider the large-scale \textit{outdoor} Aachen Day-Night v1.1~\cite{Zhang2020AachenV11} and Tokyo24/7~\cite{Torii2015Tokyo247} datasets for localization under severe illumination conditions. Image-based localization in complex \textit{indoor} environments is challenging due to the large viewpoint changes and weakly textured scenes. We use InLoc~\cite{Taira2018InLoc}, a large-scale indoor dataset with strong appearance changes between query images and the reference 3D map. The localization performance on the Aachen Day-Night v1.1 and InLoc benchmarks is reported as the percentage of correctly localized queries. For InLoc, we follow the localization pipeline\footnote{\url{https://github.com/cvg/Hierarchical-Localization}} proposed in~\cite{sarlin2019coarse, sarlin2020superglue}. The query is successfully localized if its camera position and orientation are both within a certain threshold.

The performance on the Tokyo24/7 dataset is evaluated using Recall@N, which is the number of queries that are correctly localized given $N$ nearest neighbor database images. Specifically, for a given query we first obtain a ranked list of database images, $L$ based on Euclidean distance between their global NetVLAD representations. The top-100 ranked database
images, $L^{\prime} \in L$ are re-ranked according to their similarity score based on the number of geometrically verified inliers between the query and each database image.

\customparagraph{Image retrieval.} We evaluate the proposed local image descriptors on the image retrieval benchmark. Specifically, the revisited Oxford ($\cR$Oxford5k) and revisited Paris ($\cR$Paris6k) datasets proposed by Radenovi{\'c}~\etal~\cite{Radenovic2018Revisited} have been used. Similarly to the Tokyo24/7 evaluation protocol, for each query image we first create a ranked list of database images based on cosine similarity of their global representations in the feature space and then compute
2D-2D correspondences between query and top-100 database images which are then re-ranked based on the number of inliers verified by RANSAC. To compute global descriptors, the model "retrievalSfM120k-resnet101-gem" proposed in~\cite{Radenovic2016GEM} is used. We evaluate performance by mean average precision (mAP) and mean precision at 1, 5, and 10 (mP@k), as defined by the protocol~\cite{Radenovic2018Revisited}.

\input{assets/tables/res_retrieval}



\subsection{Results}\label{ssec:results}
First, we experimentally compare the proposed models with their supervised oracles~\cite{Revaud2019R2D2,Wang2020CAPS} on the \textbf{sparse feature matching} benchmark by calculating MMA for different pixel thresholds illustrated in Figure~\ref{fig:hpatches_performance}. Following D2-Net~\cite{Dusmanu2019D2Net}, we separately report results for scenes corresponding to illumination changes (Illumination), viewpoint changes (Viewpoint), and for the whole dataset (Overall). The proposed unsupervised version of R2D2 (R2D2-U) shows a clear improvement over its supervised counterpart (R2D2-S) achieving better results for all evaluation thresholds. At the same time, although CAPS-U demonstrates competitive overall performance, it falls slightly behind its supervised baseline (CAPS-S~\cite{Wang2020CAPS}) on the illumination benchmark at larger pixel thresholds ($>$3px). Our hypothesis is that the original CAPS~\cite{Wang2020CAPS} model that leverages coarse-to-fine architecture (\cf Sec.~\ref{ssec:benchmarks_metrics}) allows to learn more discriminative descriptors leading to better matching performance. We also report homography estimation accuracy, precision (the percentage of correct matches over all the predicted matches) and recall (the ratio of correct matches over the total number of ground truth correspondences) using the same HPatches dataset. Following~\cite{Pautrat2020LISRD}, we use mutual nearest neighbor matcher and a threshold of 3 pixels to consider a match to be correct. The results are summarized in Table~\ref{tbl:hpatches_eval}. As can be seen, the proposed unsupervised models demonstrate competitive performance. Interestingly, the model utilizing global image descriptor for hard-negative mining (CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd) achieves the best Recall and Precision performance over all other methods.

\customparagraph{Visual localization.} We evaluate the performance of the proposed pipeline on the task of image-based localization. Note, that we train our approaches only on outdoor datasets,~\ie Megadepth and Phototourism but evaluate on both outdoor (Aachen v1.1) and indoor (InLoc) to test the generalization of the proposed models. We use R2D2, CAPS and R2D2* as baseline models where R2D2* represents R2D2 model trained with SuperPoint detector, \ie, the setup which is closer to our pipeline (see Sec.~\ref{sec:method}).  For unsupervised methods, we report results obtained by the models utilize in-batch hard-negative sampling during training. The percentage of correctly localized query images is presented in Table~\ref{tbl:loc_aachen_inloc}. First, if we compare R2D2-{$\left(\squarehvfill\right)$} and R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} trained on Aachen database images (A), we can notice that using only synthetic color augmentation is not sufficient to handle drastic illumination changes. Increasing the number of training samples leads to better localization performance. The model R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} trained on (M+P) is comparable to the supervised counterpart on day-time and surpasses it on night-time queries by a noticeable margin: up to $+\textbf{0.5}$ for $\left(0.5m, 5^\circ\right)$ and $+\textbf{1.1}$ for $\left(5m, 10^\circ\right)$. For indoor pose estimation, the same model can outperform the supervised baseline in all metrics: up to $+\textbf{1.5}$ and $+\textbf{2.9}$ for the finest threshold $\left(0.25m, 2^\circ\right)$ for scene DUC1 and DUC2 respectively. Leveraging visual descriptors (*-gd and *-selfgd) provides better outdoor localization results over the models trained with only stylization and color augmentations (R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} and CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}). However, in indoors, visual descriptors \textit{cannot} provide strong generalization performance leading to a marginal improvement (for the R2D2 backbone) or even poor results (with the CAPS backbone). We hypothesize that such behaviour is caused by larger gap in data distribution during training and evaluation. Interestingly, the transferring accuracy depends on the Descriptor CNN (\cf Figure~\ref{fig:pipeline_overview}) structure. The unsupervised model trained on (M+P) and based on the CAPS backbone \textit{cannot} improve performance of outdoor localization compared to its supervised baseline (CAPS~\cite{Wang2020CAPS}). However, large gains are seen for indoor setting: up to $+\textbf{6.1}$ (34.4 \textit{vs.} 40.5) for the most rigorous threshold of scene DUC2. Table~\ref{tbl:loc_tokyo247} shows the localization performance on Tokyo24/7. Similarly to the results on Aachen, R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} is \textit{better} than its supervised counterpart (R2D2-[A+R]) in all metrics: $+\textbf{1.58}$, $+\textbf{1.9}$, and  $+\textbf{1.9}$, respectively. Qualitative results of the proposed models on test images of MegaDepth are illustrated in Figure~\ref{fig:qualitative_results}.


\customparagraph{Image retrieval.} As shown in Table~\ref{tbl:image_retrieval_results}, the proposed unsupervised models show competitive image retrieval performance and surpass their supervised counterparts in mP@k and mAP on $\cR$Oxford5k and $\cR$Paris6k. Most notably, utilizing visual image descriptors with the model based on CAPS backbone leads to better retrieval accuracy which is consistent with the results obtained for the camera localizaton benchmark. However, for the R2D2 backbone model, mining harder negative samples with the help of visual descriptors leads to a marginal improvement (R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} \textit{vs.} R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd) which can be explained by the network capacity. In $\cR$Paris6k both the supervised and unsupervised methods attain comparable performance. Notably, the biggest performance improvement of 5\% is observed across mP@10 under Hard setting.

We observe that increasing the size of dataset ($A \rightarrow M \rightarrow M+P$) performs favourably on the different benchmarks. Stylization provides substantial improvements on Aachen Night time dataset, while performs comparably on other benchmarks. This indicates that the proposed network is not biased to the chosen styles. Furthermore, the proposed coarse-to-fine method with global descriptors also performs favourably compared to in-batch sampling especially on Aachen and $\cR$Oxford5k datasets. Finally, the self-supervised global mining approach *-selfgd performs comparably to *-gd which utilizes image retrieval models pre-trained on SfM data. Improving the on the fly strategy of mining hard negative local samples conditioned on visual image descriptors is a possible future direction.  %


==> hndesc_3dv2021_arXiv/sections/introduction.tex <==
\input{assets/images/fig_pipeline}

\section{Introduction}~\label{sec:introduction}
Many geometric computer vision tasks require robust estimation of local descriptors such as image alignment~\cite{Balntas2017HPatches}, structure-from-motion~\cite{heinly2015_reconstructing_the_world,schoenberger2016sfm}, image retrieval~\cite{Gordo2017Retrieval,Radenovic2018TPAMI}. With the advent of deep learning models, robust local descriptors can be learnt with highly over-parameterized networks such as Convolutional Neural Networks (CNN). Consequently, much of the latest works~\cite{Balntas2016Localdesc,Detone18superpoint,Dusmanu2019D2Net,Mishchuk2017HardNet,Revaud2019R2D2} have since focused on designing appropriate datasets, labels and loss functions to learn useful local representations.

It is well-known that CNNs are data demanding models that require large amount of data with labelled supervision. While in many cases large amount of data can be obtained, structuring it in meaningful partitions or labels is a costly process. To counter this problem, existing approaches~\cite{Gordo2017Retrieval,Radenovic2016GEM} use SfM pipelines to generate labels. Despite the effectiveness, the process incurs significant computational burden. Furthermore, integrating new stream of data to the existing dataset requires additional iterations of the costly spatial descriptor matching process. The paradigm of self-supervised learning attempts to provide a solution by enabling label-free training of CNNs. Most self-supervised methods focus on auxiliary pretext tasks~\cite{doersch_2015,noroozi_2016,zhang_2016} such as image reconstruction -- generative modelling, or discriminative optimization of the latent space based on contrastive learning~\cite{bachman_2019,dosovitskiy_2014}. The key requirement is to learn transferable representations that can adapt to downstream tasks with limited supervision. Recent progress~\cite{chen2020SimCLR,debiased,he2020moco,kalantidis,robinson_2021} in the image classification domain shows the crucial role of positives (similar) and negatives (dissimilar) in the contrastive loss function to learn robust representations. In this paper, we delve deeper into these factors for the task of local image descriptors learning.

Existing self-supervised methods for learning local descriptors~\cite{Christiansen2019Unsuperpoint,Detone18superpoint} have achieved some success by mining positives and negatives from homography related image pairs (in-pair sampling). On the other hand, \textit{supervised} local descriptor learning methods such as HardNet~\cite{Mishchuk2017HardNet} show consistent improvement with in-batch negative sampling. In addition, image retrieval methods~\cite{Gordo2017Retrieval,Radenovic2016GEM} have demonstrated remarkable results by mining global negative descriptors from a large database of thousands of images. In this paper, we propose a scalable method for sampling hard-negative local features from a wide search space that operates in a coarse-to-fine fashion by leveraging %
image descriptors.

Learning keypoint descriptors that are invariant to illumination changes is a challenging task since it is not easy to acquire suitable data. Synthetic color augmentation (CA) which is widely used to improve model robustness and performance in many computer vision applications~\cite{Fang2019InstaBoost,krizhevsky2012Imagenet,mohan2020efficientps,wu2019detectron2} can enhance illumination invariance of local descriptors only to a certain extent. Following~\cite{Revaud2019R2D2}, we propose to utilize photorealistic image stylization~\cite{Li2018Stylization} at training time. In contrast to~\cite{Revaud2019R2D2}, the more diverse style images are considered which help to increase appearance variations of our training data. We combine these findings to train existing state-of-the-art local descriptor models without any labels. During training and evaluation, only a subset of local descriptors from dense descriptors produced by the network is used. The selection is based on local keypoint detectors such as SuperPoint~\cite{Detone18superpoint} providing efficient training iterations -- by limiting hard-negative mining only to a subset of local descriptors. The proposed method is compared with strong supervised and weakly-supervised baselines~\cite{Revaud2019R2D2,Wang2020CAPS} on a wide range of benchmarks such as visual localization, sparse feature matching, and image retrieval. The key findings are analyzed and complemented by in-depth ablation study.

In summary, this work makes the following contributions: (1) we  demonstrate that improving the quality of hard negative samples during training leads to more powerful and discriminative local keypoint descriptors; (2) by leveraging visual image descriptors, we propose a coarse-to-fine method for mining hard negative local descriptors at scale; (3) we investigate several CA techniques to improve the robustness of learned feature descriptors to illumination changes and show that photorealistic image stylizations yield best performance. We demonstrate that, together, these contributions largely close the gap between self-supervised and fully-supervised approaches for feature descriptor learning. %


==> hndesc_3dv2021_arXiv/sections/method.tex <==









\section{Method}\label{sec:method}
In this section, we describe our method for local image descriptors learning that takes a single RGB image and produces a set of local feature descriptors in a self-supervised manner. Supervised methods leverage known scene geometry and utilize image- and keypoint level correspondences to increase robustness and invariance of local features to viewpoint and appearance variations. However, obtaining such ground-truth correspondence might be difficult especially for large-scale scenes. %
We analyze and carefully tailor improvements to existing self-supervised methods for learning invariant local descriptors.

We first review the main components of the proposed approach and the key ideas behind it, then we describe the hard-negative sampling procedure and training loss. An overview of our method is schematically illustrated in Figure~\ref{fig:pipeline_overview}. Given an input image $I_i \in \mathbb{R}^{H\times W\times 3}$ and a set of interest points $\mathbf{k}_i$, our goal is to predict local descriptors $\mathbf{d}_i$ corresponding to index $i$ which would be robust to appearance changes and have good generalization performance. To obtain interest points, we use SuperPoint~\cite{Detone18superpoint} detector. 

\customparagraph{Illumination Invariance}
Illumination invariance can be seen as learning context independent representations. In classification domain, various forms of CA methods such as RandAugment~\cite{Cubuk2019RandAugment} aim to remove the contextual bias in image representations. However, these methods apply various illumination transformations uniformly over both salient foreground object and background context which might be troublesome for local descriptor learning. %
Following~\cite{Melekhov2020Stylization,Revaud2019R2D2} we rely on image stylization~\cite{Li2018Stylization} to improve the robustness of local features under drastic illumination variations. Li~\etal~\cite{Li2018Stylization} propose a closed-form solution to image stylization based on a deep learning model trained in a self-supervised fashion by minimizing the sum of the reconstruction loss and perceptual loss. The method photorealistically transfers style of a reference photo to a content photo preserving local scene geometry. We use this pre-trained model as a part of our pipeline (\textbf{Style CNN} in Figure~\ref{fig:pipeline_overview}) and manually select reference images representing two style categories, \ie night and dusk, from the contributed views of the Amos Patches dataset~\cite{Pultar2019Amos}. In contrast to~\cite{Revaud2019R2D2}, for each category we consider \textit{multiple} style images which are then randomly applied to each image in the training set. The style categories and image stylization results are provided in the supplementary material.

\customparagraph{Viewpoint Invariance.} 
To model viewpoint invariance, recent self-supervised methods~\cite{Christiansen2019Unsuperpoint,Detone18superpoint}
apply a known homography transformation~\textbf{H},~\ie $\hat{I}=\mathbf{H}\left( I \right)$ followed by random crop. As in~\cite{Detone18superpoint}, we use similar types of the homographic adaptation operations: translation, rotation, perspective transform, and scale whose parameters are sampled from a uniform distribution during training (\textbf{H-crops generator}). In addition to stylization, we apply synthetic CA independently on the anchor and positive crops by adding blur, random per-pixel Gaussian noise, adaptive histogram equalization (CLAHE) along with augmentation in brightness, contrast, hue, and saturation. The full list of augmentations is also presented in supplementary.

\customparagraph{Descriptor CNN}. We use a fully-convolutional neural network architecture which takes an input crop $C_i\in \mathbb{R}^{H_c\times W_c\times 3}$ and outputs a dense map of L2-normalized fixed length descriptors, \ie $\mathbb{R}^{H_c\times W_c \times d}$. In this work, we consider two strong baseline methods (supervised and weakly-supervised), namely R2D2~\cite{Revaud2019R2D2} and CAPS~\cite{Wang2020CAPS}. Sec.~\ref{ssec:baselines} provides an overview of these baselines in more detail. In order to perform a fair comparison, we directly use R2D2 and CAPS models as a structure of Descriptor CNN.

\customparagraph{Hard-negative (HN) mining block.}
Supervised metric learning requires both positive and negative samples to learn meaningful representations. Without both positives and negatives, the model will collapse by converging to 0-valued representations. %
Existing unsupervised approaches~\cite{Detone18superpoint,Revaud2019R2D2} for learning local descriptors sample positives and negatives from a homography related image pair $\left(I, \hat{I}\right)$ with local descriptors $A \in I, P \in \hat{I}$ respectively. The images in the pair are dubbed as the anchor ($I$) and to the positive ($\hat{I}$). Each local descriptor $a_i \in A$ is associated with one $p_i \in P$ due to known homography matrix $\mathbf{H}$. Next, for each matching pair $\left(a_i, p_i\right)$ the index $n$ of the non-matching descriptor $p_n$ is obtained as follows:

\begin{equation}
    n = \argmax_{n=1..M, n\neq i} s\left(a_i, p_n\right),
\end{equation}

\noindent where $M$ is the number of interest points in $I$; $s(.)$ is a similarity function such as a dot-product. We refer to this baseline of selecting negatives as in-pair sampling. Several works~\cite{Gordo2017Retrieval,Mishchuk2017HardNet,Radenovic2016GEM} have shown that the quality of negatives has a strong impact in supervised learning of robust representations. Inspired by~\cite{Mishchuk2017HardNet}, we propose in-batch hard negatives sampling strategy that searches non-matching descriptors over all interest point embeddings $p \in B \setminus I$, where $B \sim D$ is a mini-batch sampled from the dataset $D$.

Finding the local hard negatives is an exhaustive process. Sampling negatives over a search space $D_n \sim D$ which is much larger than $B,\quad |D_n|\gg|B|$ ideally should improve the quality of negatives but incurs significant computational cost. Rather than mining hard-negatives at the local descriptor level, we propose a coarse-to-fine search method (\textbf{Image retrieval block} in Figure~\ref{fig:pipeline_overview}). For each image $I \in B$ we first find its nearest neighbor $I^n \in D_n$ in the feature space using visual descriptor $g_n$. This results in a mini-batch $B_n$ consisting of hard-negative image samples (the images look similar to the anchors $I \in B$ but \textit{not} homography related as the positives), \ie, $B_n=\{I_i^n\}_{i=1..|B|}$, which are then used to mine non-matching feature descriptors at the local level. Given the batch, $B_n$ the local descriptor pool now consists of $p_n \in B^\prime \setminus I$ where $B^\prime = (B \cup B_n)$. Such coarse-to-fine strategy leveraging visual image descriptors makes the process of mining hard-negative local descriptors tractable. Computing visual descriptors can be formulated in two ways. On the one hand, one can use state of the art image retrieval models, such as~\cite{Radenovic2016GEM,Radenovic2018TPAMI}, trained on supervised data generated by SfM systems to extract global descriptor from the entire image. On the other hand we propose a completely self-supervised approach whereby the global descriptors are constructed from the set of local descriptors extracted using the current network state. These local descriptors are then aggregated by some mean operation, such as GeM~\cite{Radenovic2016GEM}. %
Specifically, given a dense feature map $X_f \in \mathbb{R}^{H_c\times W_c \times N_d}$, visual descriptor $g_f \in \mathbb{R}^{N_d}$ is obtained by summing \textit{l2} normalized $X_f$ over the spatial resolution. The final representation is again \textit{l2} normalized.




\customparagraph{Loss functions.} Similar to~\cite{He2018LocDesc,Revaud2019R2D2}, we formulate our problem as the optimization of a differentiable approximation ($AP^\prime$) of the Average Precision (AP) ranking metric at training time:

\begin{equation}\label{eq:ap_loss}
    \mathcal{L}_{AP} = \frac{1}{N_a}\sum_i\left(1 - AP^\prime\left(a_i, p_i, \{p_{n_k}^i\}_{k=1..K}\right) \right)
\end{equation}
\noindent where $N_a$ is the number of anchor descriptors in a mini-batch $B^\prime$. In contrast to image matching~\cite{He2018LocDesc}, the number of positive and negative samples is highly imbalanced in our setting. Indeed, for each anchor descriptor in $B^\prime$ there is only one positive sample and several hundred negatives. To address this issue, we propose to select $top$-$K$ hard-negative local descriptors $\{p_{n_k}^i\}_{k=1..K}$ for $a_i$. Results presented in Sec.~\ref{ssec:results} demonstrate consistent improvement over the original AP loss~\cite{He2018LocDesc,Revaud2019R2D2}. For Triplet loss, the proposed idea of intra-batch hard-hegative mining also demonstrates better performance compared to in-pair sampling (see supplementary for more details).




==> hndesc_3dv2021_arXiv/sections/related_work.tex <==
\section{Related work}~\label{sef:related_work}
\hspace{-3mm}
\customparagraph{Local image descriptors.} Due to their generalization ability, traditional local features~\cite{Bay2006SURF,Calonder2010BRIEF,Lowe2004SIFT,Rublee2011ORB} are still popular and widely used by many existing systems where establishing pixel correspondences is essential~\cite{Labbe2019RTAB-Map,Mur2017ORB2,schoenberger2016sfm,schoenberger2016mvs}. The recent success of deep learning in various computer vision applications has motivated researchers to work on learned CNN-based approaches for interest point detection~\cite{Barroso2019KeyNet,Lenc2019Detector,Mishkin2018AffNet,Savinov2017detector,Verdie2015TILDE,zhang2017detector}, description~\cite{Balntas2016Localdesc,He2018LocDesc,Luo2019Contextdesc,Mishchuk2017HardNet,Tian2007L2Net,Tian2019SOSNET} or both detection and description~\cite{Detone18superpoint,Dusmanu2019D2Net,Germain2020S2DNet,Luo2020ASLFeat,Ono2018LFNet,Revaud2019R2D2,wang2021p2net,Yi2016LIFT}. Although, those approaches have demonstrated improved performance over classical hand-crafted methods on challenging benchmarks such as vision localization and image matching, most of them require ground-truth pixel correspondences between two views~\cite{Dusmanu2019D2Net,Jiang2021COTR,Revaud2019R2D2,Sun2021LoFTR}. Such accurate ground-truth labels are quite tedious to obtain since it requires information about the 3D representation of the scene (\eg 3D reconstruction, dense depth maps or scene flow). To address this issue, recent research directions have shifted towards weakly- and self-supervised methods. These methods rely on the supervision from epipolar geometry~\cite{Wang2020CAPS,Yang2019EPIPOLAR,Heng2019MONET,Zhou2021Patch2Pix}, principles of Reinforcement Learning~\cite{Bhowmik2020ReinforcedPoints,Truong2019GLAMpoints,Tyszkiewicz2020DISK}, relative camera poses~\cite{Bhowmik2020ReinforcedPoints,Wang2020CAPS}, camera intrinsics~\cite{Heng2021GeomPerc}, and rigid synthetic 2D transformations~\cite{Christiansen2019Unsuperpoint,Detone18superpoint,Revaud2019R2D2,tang2020NeuralRejection}. In this work, we show that with careful choices regarding hard-negative mining, color augmentation and photorealistic image stylization, we can achieve superior performance to supervised methods using only synthetic homographies. In principle, the proposed ideas can be also applied to supervised CNN-based approaches.

\customparagraph{Illumination invariance in feature descriptors.} Learning features that are invariant to illumination changes is a challenging task. To increase robustness to illumination changes, methods like~\cite{Dusmanu2019D2Net,Wang2020CAPS,Heng2021GeomPerc,Yang2020UR2KID} utilize a large SfM database of images with different lighting conditions. Domain adaptation-based methods~\cite{Anoosheh2020S2Night2Day,Mueller2019Image2Image,Porav2018Gans} utilize GANs~\cite{Goodfellow2014GANs,Zhu2017CycleGAN}, view synthesis~\cite{Mueller2019Image2Image} and few-shot learning~\cite{Baik2020DomainAdaptation} to reduce the domain gap between the training and the test (target) image distributions. Leveraging photorealistic image stylization to improve robustness to day-night variations was introduced in~\cite{Revaud2019R2D2}. In the follow-up work, Melekhov~\etal~\cite{Melekhov2020Stylization} extend the original method~\cite{Revaud2019R2D2} by considering more diverse style categories. Pautrat~\etal~\cite{Pautrat2020LISRD} propose a model predicting several dense descriptors with different levels of invariance. For a particular input image, the most relevant invariance is automatically selected using the concept of meta-descriptors based on a NetVLAD~\cite{Arandjelovic2016NetVLAD} layer. Inspired by~\cite{Melekhov2020Stylization,Revaud2019R2D2}, we utilize the idea of image stylization to improve the robustness of local descriptors to appearance variations.

\customparagraph{Self-supervised learning.} Self-supervised learning paves the way for training models on large amount of unlabelled data. Recent methods~\cite{chen2020SimCLR,he2020moco} in the classification domain are based on contrastive loss where representations from augmented copies of the original image -- positives, are contrasted against representations from other images in the batch or memory bank -- negatives. The quality of negatives was analyzed by several methods~\cite{debiased,kalantidis,robinson_2021} in improving self-supervised image representation learning. For local descriptors,~\cite{Laskar2020DensePixelMatching,dgcnet,rocco_17} consider only the augmented input image pair to sample positive and negative local descriptors (in-pair sampling). In this work, we propose methods to improve the quality of both positives and negatives. %


==> hndesc_3dv2021_arXiv_arXiv/assets/images/fig_pipeline.tex <==
\begin{figure*}[t!]
  \centering
    \includegraphics[width=\linewidth]{assets/images/raw/pipeline_small.pdf}
     \vspace{-15pt}
 \caption{\textbf{Overview of the proposed pipeline for learning local image descriptors.} Given an image and a set of interest points (top-left), we create a stylized copy of the image with a forward-pass through Style CNN. A pair of homography related crops ($c_i$) is randomly sampled from the original and stylized image in H-crops generator. We pass the image crops through Descriptor CNN to obtain representation of corresponding interest points in the feature space (embeddings). For each $a_i$ and $p_i$ descriptor from positive pair (anchors-positives), we create a list of hard-negative descriptors (shown with color gradient) using the proposed coarse-to-fine sampling procedure by leveraging global visual descriptors (Image retrieval block). Finally, the ranking loss %
 is utilized to optimize Descriptor CNN. See Sec.~\ref{sec:method} for a detailed description.}  
 \label{fig:pipeline_overview}
 \vspace{-12pt}
\end{figure*}

==> hndesc_3dv2021_arXiv_arXiv/assets/images/fig_qualitative_matches.tex <==
\begin{figure*}[t!]
  \centering
    \includegraphics[width=1\linewidth]{assets/images/raw/quality_kpts_small.pdf}
 \caption{\textbf{Qualitative matching results.} We evaluate the proposed unsupervised pipeline with two different backbone models, R2D2 (top row) and CAPS (bottom row) on test samples of the MegaDepth dataset~\cite{Li2018Megadepth}. Both models have been trained on stylized images with color augmentations using in-batch hard negative sampling. Green lines indicate correspondences estimated by RANSAC (best viewed digitally). The proposed method predicts reliable matches even without training on annotated correspondences.}
 \label{fig:qualitative_results}
\end{figure*}

==> hndesc_3dv2021_arXiv_arXiv/assets/plots/plt_mma.tex <==
\begin{figure*}[t!]
    \begin{minipage}{0.65\linewidth}
    \centering
    \includegraphics[width=\textwidth]{assets/plots/raw/hpatches_curves.pdf}
    \caption{\textbf{Mean matching accuracy (MMA) on the HPatches~\cite{Balntas2017HPatches} dataset.} For each method, the MMA with different pixel error thresholds is reported. The proposed self-supervised models (R2D2-U and CAPS-U) %
    achieve better overall performance for stricter matching thresholds (up to 3 pixels) compared to their supervised (R2D2-S and CAPS-S) counterparts. To avoid image clutter, for R2D2-U and CAPS-U, we only provide the results obtained by the {$\left(\squarehvfill,\squarerightblack\right)$} models.}
    \label{fig:hpatches_performance}
    \end{minipage}
    ~
    \begin{minipage}{0.34\linewidth}
        \centering
        \resizebox{\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{l | c c c | c c c }
		\toprule
		\multirowcell{2}{Method} & \multicolumn{3}{c|}{Illumination} & \multicolumn{3}{c}{Viewpoint} \\
		& \textEta & Precision & Recall & \textEta & Precision & Recall \\
		\midrule\midrule
		Root SIFT~\cite{Arandjelovic2012RootSIFT} & 0.933 & \textbf{0.782} & 0.799 & 0.566 & 0.651 & 0.527\\
		HardNet~\cite{Mishchuk2017HardNet} & 0.940 & 0.702 & 0.731 & 0.664 & 0.701 & 0.734\\
		SOSNet~\cite{Tian2019SOSNET} & 0.933 & 0.748 & 0.821 & \textbf{0.698} & 0.727 & 0.760\\
		SuperPoint~\cite{Detone18superpoint} & 0.912 & 0.710 & 0.811 & 0.671 & 0.685 & 0.750\\
		D2-Net~\cite{Dusmanu2019D2Net} & 0.905 & 0.725 & 0.775 & 0.617 & 0.666 & 0.664\\
		LISRD~\cite{Pautrat2020LISRD} & \textbf{0.947} & 0.766 & 0.920 & 0.688 & 0.731 & 0.757\\
		\textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & 0.940 & 0.762 & 0.837 & 0.692 & 0.720 & 0.732\\
		\textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & 0.888 & 0.757 & \textcolor{Cyan}{\underline{\textbf{0.938}}} & \textcolor{Cyan}{\underline{0.692}} & 0.723 & 0.699\\
		\midrule\midrule
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & 0.944 & 0.764 & \textcolor{Magenta}{\underline{0.838}} & 0.678 & \textcolor{Magenta}{\underline{0.732}} & \textcolor{Magenta}{\underline{0.739}} \\
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & 0.933 &	0.761 &	0.817 &	0.678 &	0.715 &	0.705  \\
		R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & \textcolor{Magenta}{\underline{\textbf{0.947}}} &	\textcolor{Magenta}{\underline{0.766}}	& 0.826 &	\textcolor{Magenta}{\underline{\textbf{0.698}}} &	0.726 &	0.720 \\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & 0.933 & 0.750 & 0.884 & 0.671 & 0.742 & 0.728 \\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & \textcolor{Cyan}{\underline{0.937}} &	0.756 &	0.893 &	0.661 &	0.740 &	0.752\\
		CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & 0.919 & \textcolor{Cyan}{\underline{0.757}} & 0.890 & 0.681 & \textcolor{Cyan}{\underline{\textbf{0.747}}} & \textcolor{Cyan}{\underline{\textbf{0.762}}}\\
		\end{tabular}}
		\captionof{table}{\textbf{Evaluation results on HPatches.} We follow~\cite{Pautrat2020LISRD} and report the accuracy of homography estimation, precision and recall for error thresholds of 3 pixels. The best score between supervised baselines, \textcolor{Magenta}{R2D2} and \textcolor{Cyan}{CAPS}, and the proposed methods for each category is \underline{underlined}. The overall best score is in \textbf{bold}.}\label{tbl:hpatches_eval}
    \end{minipage}
    
\end{figure*}


==> hndesc_3dv2021_arXiv_arXiv/assets/tables/ablation_all.tex <==
\begin{table}[t!]
    \begin{subtable}[t]{0.49\textwidth}
        \begin{center}
	    \resizebox{0.9\textwidth}{!}{%
		\footnotesize 		
		\begin{tabular}{c c c | c c }
		\toprule 
		\multirow{2}{*}{} & \multicolumn{2}{c|}{\multirowcell{2}{Metric}} & \multicolumn{2}{c}{Negative sampling type} \\
		& & & in-pair & in-batch \\ \midrule\midrule
		\multirow{4}{*}{\rotatebox[origin=c]{90}{$\cR$Oxford5k}} & \multirowcell{2}{mAP} & M & 55.38 & \textbf{58.69} \\
		& & H & 29.67 & \textbf{33.17} \\ \cmidrule{2-5}
		& \multirowcell{2}{mP@k $[1, 5, 10]$} & M & [94.29,	86.57, 78.43] & [\textbf{95.71}, \textbf{89.71}, \textbf{83.29}]\\
		& & H & [82.86, 54.57, 42.29] & [\textbf{85.71}, \textbf{60.29}, \textbf{45.71}]
        \\ \midrule\midrule
		\multirow{3}{*}{\rotatebox[origin=c]{90}{HPatches}} & \multirowcell{3}{MMA} & 1px & 0.239 / 0.425 / 0.332 & \textbf{0.254} / \textbf{0.439} / \textbf{0.346} \\
		& & 3px & 0.585 / 0.677 / 0.631 & \textbf{0.630} / \textbf{0.707} / \textbf{0.669} \\
		& & 5px & 0.648 / 0.742 / 0.695 & \textbf{0.706} / \textbf{0.784} / \textbf{0.745} \\[2pt] \midrule \midrule
		
		\multirow{2}{*}{\rotatebox[origin=c]{90}{Aachen}} &  & day & 87.9 / 94.2 / 97.9 &	\textbf{88.2} / \textbf{95.5} / \textbf{98.7} \\[1pt]
		& & night & 66.5 / 79.1 / 91.6 & \textbf{68.1} / \textbf{83.8} / \textbf{94.8} 
        \\[3pt] \midrule
        \end{tabular}
        }
	\end{center}
	\vspace{-15pt}
	\caption{\textbf{In-batch} \textit{vs.} \textbf{in-pair} hard negative sampling. Intra-batch negative mining performs consistently better over in-pair counterpart in all metrics. }\label{tbl:ablation_batch_vs_pair}
    \end{subtable}
        
    \begin{subtable}[h]{.49\textwidth}
        	\begin{center}
	\resizebox{0.9\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c c c | c | c c c }
		\toprule
		\multirow{2}{*}{} & \multicolumn{2}{c|}{\multirowcell{2}{Metric}} & \multirowcell{2}{Baseline} & \multicolumn{3}{c}{Negative samples in mini-batch} \\
		& & & & $all$ & $random$ & $top$-$k$ \\ \midrule\midrule
		\multirow{12}{*}{\rotatebox[origin=c]{90}{$\cR$Oxford5k}} & \multirowcell{3}{mAP} & E & $72.60$ & \underline{72.85} & $72.06$ & $\textbf{75.27}$ \\
		& & M & $54.89$ & \underline{57.06} & $56.91$ & $\textbf{57.83}$ \\
		& & H & $27.37$ & \underline{30.53} & $31.28$ & $\textbf{31.56}$ \\ \cmidrule{2-7}
		& \multirowcell{9}{mP@k $[1, 5, 10]$} & \multirowcell{3}{E} & $94.12$	& $\textbf{97.06}$ &	\underline{95.59} & $\textbf{97.06}$ \\
		& & & $80.74$ & $84.41$ & \underline{84.63} & $\textbf{88.24}$ \\
		& & & $74.12$ & $77.40$ & \underline{77.72} & $\textbf{80.44}$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{M} & $91.43$ & $\textbf{95.71}$ & $94.29$ & $\textbf{95.71}$ \\
		& & & $80.57$ & \underline{88.10} & $\textbf{88.86}$ & $\textbf{88.86}$ \\
		& & & $73.86$ & \underline{81.24} & $81.00$ & $\textbf{81.41}$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{H} & $61.43$ & \underline{81.43} & \underline{81.43} & $\textbf{82.86}$ \\
		& & & $47.50$ & $56.43$ & \underline{57.14} & $\textbf{59.43}$ \\
		& & & $39.79$ & $43.57$ & \underline{44.57} & $\textbf{45.43}$ \\ \midrule\midrule
		\multirowcell{3}{\rotatebox[origin=c]{90}{ Tokyo24/7}} & \multirowcell{3}{recall} & r@1 & $67.10$ & \underline{76.15} & $74.92$ & $\textbf{79.05}$ \\[2pt]
		& & r@5 & $74.20$ & \underline{81.27} & $80.63$ & $\textbf{84.13}$ \\[2pt]
		& & r@10 & $76.10$ & \underline{83.49} & $81.90$ & $\textbf{85.71}$ \\[2pt] \midrule
		\multirow{6}{*}{\rotatebox[origin=c]{90}{Aachen v1.1}} & \multirowcell{6}{$0.25m, 2^\circ$ \\ $0.5m, 5^\circ$ \\ $5m, 10^\circ$} & \multirowcell{3}{day} & \underline{87.7} & $87.5$ & $88.0$ & $\textbf{88.0}$ \\
		& & & \underline{94.7} & $94.4$ & 94.2 & $\textbf{94.8}$ \\
		& & & \textbf{98.7} & \underline{98.3} & $98.1$ & $98.2$ \\ \cmidrule{3-7}
		& & \multirowcell{3}{night} & \underline{69.6} & $\textbf{70.2}$ & $67.0$ & $\textbf{70.2}$ \\
		& & & \textbf{86.4} & \underline{85.9} & 84.3 & \textbf{86.4} \\
		& & & \underline{95.3} & \textbf{95.8} & $94.8$ & \textbf{95.8} \\ \midrule
		\multirow{6}{*}{\rotatebox[origin=c]{90}{InLoc}} & \multirowcell{6}{$0.25m, 2^\circ$ \\ $0.5m, 5^\circ$ \\ $5m, 10^\circ$} & \multirowcell{3}{DUC1} & \underline{27.8} & \textbf{28.3} & 27.3 & \underline{27.8}  \\
		& & & 42.4 & \textbf{46.0} & 43.4 & \underline{43.9} \\
		& & & \underline{54.4} & \textbf{55.6} & 53.0 & 54.0 \\ \cmidrule{3-7}
		& & \multirowcell{3}{DUC2} & 22.1 & 23.7 & \underline{26.0} & \textbf{27.5} \\
		& & & 34.4 & 35.1 & \underline{36.6} & \textbf{38.2} \\
		& & & 42.7 & 40.5 & \underline{44.3} & \textbf{49.6} \\ \midrule
		\end{tabular}
		
	}
	
	\end{center}
	\vspace{-15pt}
	\caption{\textbf{Intra-batch negative sampling}. For a listwise loss, the $top$-$k$ sampling strategy leads to a better performance over its counterparts in almost all metrics. The best score is in bold and the second best score is underlined.}\label{tbl:ablation_topK_vs_all}
    \end{subtable}
    \vspace{-5pt}
    \caption{\textbf{Ablation study.} We analyze the influence of different design choices of the proposed approach. See Sec.~\ref{sec:ablation} for more details.}
    \vspace{-15pt}
\end{table}


==> hndesc_3dv2021_arXiv_arXiv/assets/tables/res_localization_all.tex <==
\begin{table*}[t!]
    \begin{subtable}[h]{0.7\textwidth}
        \begin{center}
	    \resizebox{\textwidth}{!}{%
		\footnotesize 		
		\begin{tabular}{c l | c c | c c c | c c c | c c c | c c c}
		\toprule
		\multirow{4}{*}{} & \multirowcell{4}{Method} & \multirowcell{4}{Supervision} & \multirowcell{4}{Training\\data} & \multicolumn{6}{c}{Aachen v1.1} & \multicolumn{6}{|c}{InLoc} \\
		& & & & \multicolumn{6}{c}{\% localized queries} & \multicolumn{6}{|c}{\% localized queries} \\
		& & & & \multicolumn{3}{c|}{Day (824 images)} & \multicolumn{3}{c}{Night (191 images)} & \multicolumn{3}{|c|}{DUC1} &  \multicolumn{3}{c}{DUC2} \\
		& & & & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ & $0.25m, 2^\circ$ & $0.5m, 5^\circ$ & $5m, 10^\circ$ \\ \midrule\midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Super}} & \textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & OF & A+R & \textcolor{Magenta}{\textbf{88.6}} & \textcolor{Magenta}{\textbf{95.4}} & \textcolor{Magenta}{\textbf{98.9}} & 72.8 & 89.0 & 97.4 & 27.8 & 42.4 & 54.5 & 22.1 & 34.4 & 42.7 \\
        & \textcolor{Magenta}{R2D2*} & OF & A & 87.7 & 94.7 & 98.7 & 69.6 & 86.4 & 95.3 & 29.8 & 43.4 & 55.1 & 21.4 & 34.4 & 43.5 \\
        & \textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & SL+RP & M & 85.3 & \textcolor{Cyan}{\textbf{93.8}} & 97.9 & \textcolor{Cyan}{\textbf{75.9}} & 88.5 & \textcolor{Cyan}{\textbf{97.9}} & 38.4 & 59.1 & \textcolor{Cyan}{\textbf{74.7}} & 34.4 & 52.7 & 61.8\\ \midrule\midrule
        \multirow{11}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-$\left(\squarehvfill\right)$ & - & A & 87.4 & 94.9 & 98.3 & 63.9 & 80.1 & 92.1 & \textcolor{Magenta}{\textbf{29.3}} & 46.5 & 57.6 & 29.8 & 42.0 & 51.1 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & A & 88.0 & 94.8 & 98.2 & 70.2 & 86.4 & 95.8 & 27.8 & 46.5 & 57.6 & 29.8 & 42.0 & 51.1\\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M & 87.4 & 94.7 & 98.3 & 72.3 & 88.5 & 97.4 & 26.8 & 46.0 & 57.1 & 26.7 & \textcolor{Magenta}{\textbf{42.7}} & 48.9 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & - & M & 87.5 & 94.9 & 98.3 & 71.7 & 86.4 & 96.9 & 27.8 & 43.4 & 54.5 & 28.2 & 41.2 & 51.9 \\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & - & M & 88.1 & 94.8 & 98.1 & 71.2 & 88.0 & 95.8 & 30.8 & 43.9 & 54.0 & 28.2 & 37.4 & 46.6\\
        & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M+P & 88.2 & 95.1 & 98.5 & \textcolor{Magenta}{\textbf{73.3}} & \textcolor{Magenta}{\textbf{90.1}} & \textcolor{Magenta}{\textbf{97.4}} & \textcolor{Magenta}{\textbf{29.3}} & \textcolor{Magenta}{\textbf{47.0}} & \textcolor{Magenta}{\textbf{58.1}} & \textcolor{Magenta}{\textbf{25.2}} & 41.2 & \textcolor{Magenta}{\textbf{51.9}} \\ 
        \cmidrule{2-16}
        & CAPS-{$\left(\squarehvfill\right)$} & - & M & 85.8 & 93.8 & 98.2 & 67.0 & 82.2 & 96.9 &35.9 & 54.0 & 69.2 & 38.9 & 50.4 & 64.9\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M & 85.1 & 93.2 & 97.8 & 71.7 & 87.4 & \textcolor{Cyan}{\textbf{97.9}} & \textcolor{Cyan}{\textbf{39.9}} & \textcolor{Cyan}{\textbf{61.6}} & 70.7 & 38.2 & 51.1 & \textcolor{Cyan}{\textbf{66.4}}\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & - & M & \textcolor{Cyan}{\textbf{87.0}} & \textcolor{Cyan}{\textbf{93.8}} & \textcolor{Cyan}{\textbf{98.3}} & 73.8 & \textcolor{Cyan}{\textbf{89.0}} & 97.4 & 35.9 & 53.0 & 65.7 & 32.8 & 47.3 & 61.1\\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & - & M & 86.9 & \textcolor{Cyan}{\textbf{93.8}} & 98.1 & 71.7 & \textcolor{Cyan}{\textbf{89.0}} & 97.4 & 35.9 & 53.5 & 64.6 & 30.5 & 45.0 & 58.8 \\
        & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & - & M+P & 85.4 & 93.2 & 97.9 & 72.3 & 88.5 & \textcolor{Cyan}{\textbf{97.9}} & 38.9 & 56.1 & 69.2 & \textcolor{Cyan}{\textbf{40.5}} & \textcolor{Cyan}{\textbf{54.2}} & \textcolor{Cyan}{\textbf{66.4}}\\
		\end{tabular}
        }
	\end{center}
	\vspace{-5pt}
	\caption{Evaluations results for Aachen v1.1~\cite{Zhang2020AachenV11} and InLoc~\cite{Taira2018InLoc} }\label{tbl:loc_aachen_inloc}
    \end{subtable}
    ~
    \begin{subtable}[h]{.29\textwidth}
        	\begin{center}
	\resizebox{.9\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c l|l l l}
        \multirow{2}{*}{} & \multirow{2}{*}{Method} & \multicolumn{3}{|c}{Recall} \\
        & & \multicolumn{1}{|c}{r@1} & \multicolumn{1}{c}{r@5} & \multicolumn{1}{c}{r@10}\\
    \hline
    \hline
    & DenseVLAD~\cite{Torii2015Tokyo247} & 67.10 & 74.20 & 76.10 \\
    & NetVLAD-TokyoTM~\cite{Arandjelovic2016NetVLAD} & 71.10 & 83.10 & 86.20 \\
    & SIFT~\cite{Lowe2004SIFT} & 73.33 & 80.00 & 84.40 \\
    & InLoc~\cite{Taira2018InLoc} & 62.54 & 67.62  & 70.48 \\
    & Dense Pixel Matching~\cite{Laskar2020DensePixelMatching} & 77.14 & 84.44 & 86.67 \\
    & \textcolor{Magenta}{R2D2}-[A+R]~\cite{Revaud2019R2D2} & 78.10 & 82.54 & 84.13 \\
    & \textcolor{Cyan}{CAPS}-[M]~\cite{Wang2020CAPS} & \textcolor{Cyan}{\textbf{83.49}} & 86.67 & 87.94 \\ \hline \hline
    \multirow{9}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[A] & 79.05 & 83.17 & 85.71 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[M] & 79.37 & \textcolor{Magenta}{\textbf{84.76}} & 85.71 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd-[M] & 78.41 & 82.54 & 83.81 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd-[M] & 77.78 & 82.86 & 85.40 \\
    & R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-[M+P] & \textcolor{Magenta}{\textbf{79.68}} & 84.44 & \textcolor{Magenta}{\textbf{86.03}} \\ \cmidrule{2-5}
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-[M] & 82.54 & 86.03 & 87.94 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd-[M] & 81.27 & 85.71 & 86.98 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd-[M] & 82.54 & 86.35 & 87.94 \\
    & CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-[M+P] & 82.86 & \textcolor{Cyan}{\textbf{87.30}} & \textcolor{Cyan}{\textbf{88.25}} \\

    \end{tabular}
		
	}
	
	\end{center}
	\vspace{-10pt}
	\caption{Performance on Tokyo24/7~\cite{Torii2015Tokyo247}}\label{tbl:loc_tokyo247}
    \end{subtable}
    
    \vspace{-5pt}
    \caption{\textbf{Indoor and outdoor localization performance}. The supervised baseline methods, \textcolor{Magenta}{R2D2} and \textcolor{Cyan}{CAPS}, are color-coded. Best results in each category for each localization benchmark are in \textbf{bold}. \textbf{Legend}: \textit{Supervision}: OF~--~ground-truth pixel correspondences based on optical flow~\cite{Revaud2019R2D2}; SL~--~ground-truth scene labels; RP~--~relative camera poses. \textit{Training data}: A~--~Aachen database images; R~--~Random images from the Internet~\cite{Revaud2019R2D2}; M~--~MegaDepth dataset; P~--~Phototourism dataset. For Tokyo24/7, the training datasets for our supervised baselines and the proposed approach are given in $\left[.\right]$ parentheses.}
    
\end{table*}


==> hndesc_3dv2021_arXiv_arXiv/assets/tables/res_retrieval.tex <==
\begin{table*}[t!]
	\begin{center}
	\resizebox{.99\textwidth}{!}{%
		\footnotesize
		\begin{tabular}{c l | c c | c c c | c c c | c c c | c c c | c c c |  c c c | c c c | c c c}
		\toprule
		 \multirow{3}{*}{} & \multirowcell{3}{Method} & \multirowcell{3}{Training\\data} & \multirowcell{3}{Hard-negative\\mining} & \multicolumn{12}{|c}{$\cR$Oxford5k} & \multicolumn{12}{|c}{$\cR$Paris6k} \\
	     & & & & \multicolumn{3}{c}{mAP} & \multicolumn{9}{|c|}{mP@k [1, 5, 10]} & \multicolumn{3}{c}{mAP} & \multicolumn{9}{|c}{mP@k [1, 5, 10]} \\
		 & & & & E & M & H & \multicolumn{3}{c|}{E} & \multicolumn{3}{c|}{M} & \multicolumn{3}{c|}{H} & E & M & H & \multicolumn{3}{c|}{E} & \multicolumn{3}{|c|}{M} &  \multicolumn{3}{c}{H} \\ \midrule\midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{Supervised}} & Baseline~\cite{Radenovic2016GEM} & - & - & 72.60 & 54.89 &	27.37 & 91.43 & 80.74 & 74.12 & 91.43 & 80.57 & 73.86 & 61.43 & 47.50 & 39.79 & 86.15 & 68.98 & 43.86 & 98.57 & 95.14 & 93.43 & 98.57 & 98.57 & 96.14 & 95.71 & 87.71 & 82.86\\
		& \textcolor{Magenta}{R2D2}~\cite{Revaud2019R2D2} & A+R & in-pair & 76.39 & \textcolor{Magenta}{\textbf{59.09}} & \textcolor{Magenta}{\textbf{33.20}} & 97.06 & 88.38 & 81.55 & 95.71 & 89.71 & 83.57 & \textcolor{Magenta}{\textbf{85.71}} & \textcolor{Magenta}{\textbf{61.14}} & \textcolor{Magenta}{\textbf{47.14}} & 85.73 & 68.51 & 42.86 & \textcolor{Magenta}{\textbf{100}} & 97.24 & 95.81 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{100}} & 99.14 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{92.57}} & 81.57\\
		& R2D2* & A & in-pair & 75.36 & 58.61 & 32.69 & 97.06 & 87.35 & 79.56 & 95.71 & 89.43 & 82.57 & 85.71 & 59.14 & 45.86 & 85.39 & 68.36 & 42.93 & 100 & 97.43 & 96.14 & 100 & 99.71 & 98.86 & 98.57 & 91.14 & 82.43\\
        & \textcolor{Cyan}{CAPS}~\cite{Wang2020CAPS} & M & - & 75.27 & 59.67 & \textcolor{Cyan}{\textbf{34.77}} & 94.12 & 86.76 & 80.44 & 94.29 & 89.14 & 84.14 & \textcolor{Cyan}{\textbf{85.71}} & \textcolor{Cyan}{\textbf{66.00}} & \textcolor{Cyan}{\textbf{50.57}} & \textcolor{Cyan}{\textbf{88.92}} & \textcolor{Cyan}{\textbf{69.87}} & \textcolor{Cyan}{\textbf{44.47}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{99.43}} & \textcolor{Cyan}{\textbf{97.43}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 98.57 & \textcolor{Cyan}{\textbf{94.86}} & \textcolor{Cyan}{\textbf{87.14}}\\ \midrule\midrule
		& R2D2-$\left(\squarehvfill\right)$ & M & in-pair & 70.99 & 55.38 & 29.67 & 95.59 & 84.12 & 75.44 & 94.29 & 86.57 & 78.43 & 82.86 & 54.57 & 42.29 & 84.57 & 67.95 & 42.57 & 100 & 97.14 & 96.00 & 100 & 100 & 99.14 & 100 & 90.29 & 81.86  \\
        \multirow{8}{*}{\rotatebox[origin=c]{90}{Self-supervised}} & R2D2-$\left(\squarehvfill\right)$ & A & in-batch & 73.16 & 56.47 & 30.05 & 95.59 & 85.51 & 77.87 & 94.29 & 87.14 & 79.29 & 82.86 & 55.43 & 42.57 & 86.09 & 68.60 & \textcolor{Magenta}{\textbf{43.04}} & 100 & 98.00 & 96.43 & 100 & 99.71 & 99.43 & 97.14 & 91.71 & \textcolor{Magenta}{\textbf{82.71}}  \\
		& R2D2-$\left(\squarehvfill\right)$ & M & in-batch & 75.09 & 58.69 & 33.17 & 97.06 & 87.06 & 80.15 & 95.71 & 89.71 & 83.29 & 85.71 & 60.29 & 45.71 & 86.38 & 68.60 & 42.83 & 100 & 98.00 & \textcolor{Magenta}{\textbf{96.86}} & 100 & 100 & \textcolor{Magenta}{\textbf{99.57}} & 98.57 & 91.43 & 82.57 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & M & in-batch & 75.70 & 58.79 & 33.03 & 97.06 & 86.57 & 80.88 & 95.71 & 89.14 & 82.57 & 88.57 & 60.00 & 46.29 & 86.49 & 68.67 & 42.86 & 100 & 98.29 & 96.43 & 100 & 100 & 99.29 & \textcolor{Magenta}{\textbf{100}} & 92.00 & 82.14 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & M & in-batch & 75.97 & 58.70 & 32.85 & 97.06 & 88.24 & 81.03 & 95.71 & \textcolor{Magenta}{\textbf{90.00}} & 83.14 & 85.71 & 60.29 & 46.86 & 86.31 & 68.63 & 42.85 & 100 & 98.00 & 96.29 & 100 & 100 & 99.43 & 100 & 91.14 & \textcolor{Magenta}{\textbf{82.71}} \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & M & in-batch & 73.47 & 57.57 & 32.16 & 97.06 & 85.59 & 76.91 & 95.71 & 88.86 & 81.29 & 85.71 & 58.57 & 46.43 & 86.04 & 68.48 & 42.76 & 100 & 97.71 & 96.14 & 100 & 99.71 & 99.29 & 98.57 & 89.71 & 82.29 \\
		& R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} & M+P & in-batch & \textcolor{Magenta}{\textbf{76.65}} & 59.07 & 33.15 & \textcolor{Magenta}{\textbf{97.06}} & \textcolor{Magenta}{\textbf{88.82}} & \textcolor{Magenta}{\textbf{81.62}} & \textcolor{Magenta}{\textbf{95.71}} & 89.43 & \textcolor{Magenta}{\textbf{83.71}} & \textcolor{Magenta}{\textbf{85.71}} & 60.57 & \textcolor{Magenta}{\textbf{47.14}} & \textcolor{Magenta}{\textbf{87.02}} & \textcolor{Magenta}{\textbf{68.80}} & 42.85 & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{98.57}} & \textcolor{Magenta}{\textbf{96.86}} & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{100}} & \textcolor{Magenta}{\textbf{99.57}} & 98.57 & 91.43 & 81.86 \\ \cmidrule{2-28}
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & M & in-batch & 74.68 & 58.64 & 32.54 & 95.59 & 87.06 & 78.38 & 94.29 & 89.71 & 82.71 & 82.86 & 59.14 & 46.29 & 87.88 & 69.25 & 43.46 & 100 & 99.14 & 96.71 & 100 & 100 & 99.71 & 100 & 92.86 & 84.14 \\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd & M & in-batch & 77.06 & 59.67 & 32.89 & 95.59 & 88.82 & \textcolor{Cyan}{\textbf{82.04}} & 94.29 & 90.57 & \textcolor{Cyan}{\textbf{84.71}} & 82.86 & 60.00 & 47.57 & 87.36 & 69.19 & 43.54 & 100 & 98.86 & 96.71 &  100 & 100 & 99.86 & 100 & 94.00 & 84.71 \\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-selfgd & M & in-batch & \textcolor{Cyan}{\textbf{77.17}} & 59.54 & 32.71 & \textcolor{Cyan}{\textbf{97.06}} & \textcolor{Cyan}{\textbf{89.85}} & 81.47 & \textcolor{Cyan}{\textbf{95.71}} & \textcolor{Cyan}{\textbf{90.86}} & 84.43 & \textcolor{Cyan}{\textbf{85.71}} & 60.57 & 47.29 & 87.61 & 69.14 & 43.33 & \textcolor{Cyan}{\textbf{100}} & 98.86 & 96.71 & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 99.57 & \textcolor{Cyan}{\textbf{100}} & 93.43 & 83.71\\
		& CAPS-{$\left(\squarehvfill,\squarerightblack\right)$} & M+P & in-batch & 76.49 & \textcolor{Cyan}{\textbf{59.72}} & 33.60 & 95.59 & 88.16 & 81.54 & 94.29 & 89.71 & 84.14 & 84.29 & 62.00 & 48.14 & 87.66 & 69.12 & 43.34 & \textcolor{Cyan}{\textbf{100}} & 98.86 & 97.00 & \textcolor{Cyan}{\textbf{100}} & \textcolor{Cyan}{\textbf{100}} & 100 & 100 & 93.14 & 84.71\\
		\end{tabular}
	}
	\caption{\textbf{Image retrieval performance}. We report results for the $\cR$Oxford5k and $\cR$Paris6k datasets following the evaluation protocol proposed in~\cite{Radenovic2018Revisited}. We use the same color-map for the supervised baseline approaches as in Table~\ref{tbl:loc_aachen_inloc}. The proposed unsupervised models demonstrate competitive performance 
	\vspace{-5mm}
	\label{tbl:image_retrieval_results}}
	\end{center}

\end{table*}


==> hndesc_3dv2021_arXiv_arXiv/sections/ablation.tex <==
\section{Ablation Study}\label{sec:ablation}
The goal of this section is to investigate the benefits of using intra-batch hard negative mining compared to in-pair sampling used in recent CNN-based interest point detectors and descriptors~\cite{Dusmanu2019D2Net,Revaud2019R2D2}. For in-batch negative mining, we experiment with different sampling strategies: consider \textit{all} negative samples in a mini-batch, take $k$ negative samples \textit{randomly}, and consider only $top$-$k$ samples.

\customparagraph{In-pair \textit{vs.} in-batch negative mining.} To evaluate the effectiveness of the sampling procedure we conduct controlled experiments summarized in Table~\ref{tbl:ablation_batch_vs_pair}. The results are obtained by the R2D2-{$\left(\squarehvfill\right)$} model trained on the MegaDepth dataset using the AP loss function. We use the following evaluation benchmarks: sparse feature matching (HPatches), image retrieval ($\cR$Oxford5k), and visual localization (Aachen v1.1) (see Sec.~\ref{ssec:benchmarks_metrics}). As shown in Table~\ref{tbl:ablation_batch_vs_pair}, in-batch hard-negative sampling significantly outperforms in-pair mining in all metrics. We observe similar behaviour with metric learning losses, \eg, Triplet loss. The results obtained by models trained with Triplet loss are provided in supplementary.

\customparagraph{In-batch sampling: all \textit{vs.} random \textit{vs.} topK.} In contrast to \textit{pairwise} ranking losses, the AP loss is defined on a ranked list of samples $L$. Let us assume we have a mini-batch consisting of $M$ homography related image crop pairs where each crop has $p$ interest points extracted by SuperPoint~\cite{Detone18superpoint} detector. Each keypoint is associated with a feature vector and has one positive and $M\times(p-1)$ negative samples within a mini-batch. Therefore, we consider 3 ways of constructing the list $L$: take all possible negatives, randomly select $k$ samples from $M\times(p-1)$, and select $top$-$k$ negatives (the proposed strategy). For each setting, we train our unsupervised R2D2-{$\left(\squarehvfill\right)$} model on (A) and evaluate on two benchmarks: image retrieval and image-based localization. The results are presented in Table~\ref{tbl:ablation_topK_vs_all}. The proposed "top-k negative" sampling approach surpasses its counterparts with a noticeable margin. The number of hard negative samples $k$ is set to 30 after empirical evaluation for all our experiments. Interestingly, unlike Triplet loss~\cite{Mishchuk2017HardNet}, the AP loss with random sampling will \textit{not} lead to overfit, but evaluation performance is low.


\input{assets/tables/ablation_all}

==> hndesc_3dv2021_arXiv_arXiv/sections/abstract.tex <==
Fully-supervised CNN-based approaches for learning local image descriptors have shown remarkable results in a wide range of geometric tasks. However, most of them require per-pixel ground-truth keypoint correspondence data which is difficult to acquire at scale. To address this challenge, recent weakly- and self-supervised methods can learn feature descriptors from relative camera poses or using only synthetic rigid transformations such as homographies. In this work, we focus on understanding the limitations of existing self-supervised approaches and propose a set of improvements that combined lead to powerful feature descriptors. We show that increasing the search space from in-pair to in-batch for hard negative mining brings consistent improvement. To enhance the discriminativeness of feature descriptors, we propose a coarse-to-fine method for mining local hard negatives from a wider search space by using global visual image descriptors. We demonstrate that a combination of synthetic homography transformation, color augmentation, and photorealistic image stylization produces useful representations that are viewpoint and illumination invariant. The feature descriptors learned by the proposed approach perform competitively and surpass their fully- and weakly-supervised counterparts on various geometric benchmarks such as image-based localization, sparse feature matching, and image retrieval. 








==> hndesc_3dv2021_arXiv_arXiv/sections/conclusion.tex <==
\section{Conclusion}
In this work, we have presented a self-supervised local descriptor learning framework. We introduced three main contributions: (1) a coarse-to-fine method to efficiently sample hard-negative local descriptors by leveraging visual image descriptors, (2) the modified version of AP loss which can carefully handle imbalance between the number of positive and negative keypoint descriptors and (3) photorealistic image stylization that combined with synthetic color augmentation can significantly enhance the robustness of learned local descriptors to illumination changes. The proposed improvements together result in a self-supervised approach demonstrates favourable performance on a wide range of geometric tasks compared to strong fully- and weakly-supervised baseline models.



==> hndesc_3dv2021_arXiv_arXiv/sections/experiments.tex <==
\section{Experiments} \label{sec:experiments_results}
Here, we describe the experimental setting and validate that (1) increasing the search space from within-pair to intra-batch for hard negative mining improves the discriminativeness of local image descriptors and leads to better performance, (2) photorealistic image stylization in addition to color augmentations demonstrates good generalization performance and improves results, especially when query images are taken during challenging illumination conditions, (3) self-supervised methods for local image descriptors learning achieve competitive results with their fully- and weakly-supervised counterparts. In order to highlight the effectiveness of the proposed ideas, we further present an extensive ablation study.

\input{assets/plots/plt_mma}

\subsection{Baselines}\label{ssec:baselines}
In this work, we consider two recent approaches, R2D2~\cite{Revaud2019R2D2} and CAPS~\cite{Wang2020CAPS}, as the baseline methods. Since we focus exclusively on local image descriptors learning, SuperPoint~\cite{Detone18superpoint} keypoint detector is used in all our experiments and the baselines.

\customparagraph{R2D2}~\cite{Revaud2019R2D2} can directly extract dense descriptors and a heatmap of keypoints from an input image. It consists of L2-Net backbone network with two heads for jointly learning repeatable and reliable matches. The network was trained on pairs of image crops with known pixel correspondences based on either synthetic homography or 3D reprojection. We consider the model trained with 3D supervision as our baseline.

\customparagraph{CAPS}~\cite{Wang2020CAPS} is a CNN-based local image descriptor trained in a weakly-supervised manner. Specifically, it can learn feature descriptors using only scene labels and relative camera poses between views. It utilizes SuperPoint keypoints and an epipolar constraint on pixel locations of matched points as a supervision signal. The resulting descriptor consists of two concatenated 128-dimensional feature vectors, \ie coarse- and fine-level descriptors, extracted at different parts of the model encoder (an ImageNet-pretrained ResNet-50 architecture~\cite{Deng2009ImageNet,He2016ResNet}). In our experiments, we utilize \textit{only} fine-level descriptors to optimize the proposed criterion (Eq.~\ref{eq:ap_loss}).



\input{assets/images/fig_qualitative_matches}

\input{assets/tables/res_localization_all}

\subsection{Notations}\label{ssec:notations}
We use the following symbolic notation throughout the paper: {$\left(\squarehvfill\right)$} denotes models trained with synthetic CA; {$\left(\squarerightblack\right)$} indicates photorealistic stylized images; {$\left(\squarehvfill,\squarerightblack\right)$} if both CA and style transfer are used during training. Finally, we refer the models utilizing image retrieval pre-trained networks for extracting visual descriptors with a suffix~\texttt{*-gd} and~\texttt{*-selfgd} denotes the self-supervised way of computing visual descriptors on the fly using the current state of the proposed Descriptor CNN (\cf Figure~\ref{fig:pipeline_overview}).


\subsection{Benchmarks and metrics}\label{ssec:benchmarks_metrics}
We verify the proposed ideas on the following benchmarks.

\customparagraph{Sparse feature matching.} For this experiment, we evaluate our descriptors on the full images provided by the HPatches dataset~\cite{Balntas2017HPatches}. The dataset consists of 116 image sequences with varying photometric and viewpoint changes. Each sequence contains a reference image and 5 source images taken under a different viewpoint. For all image pairs, the estimated ground-truth homography matrix with respect to the reference image is provided. We follow the standard evaluation protocol~\cite{Dusmanu2019D2Net} and use the mean matching accuracy (MMA) as the metric, \ie the average percentage of correct matches per image under a certain pixel threshold. In addition to MMA, we also report a homography estimation score~\cite{Detone18superpoint,Dusmanu2019D2Net}, precision and recall computed for a 3-pixel error threshold. %

\customparagraph{Image-based localization.} To verify the generalization performance of the proposed approach, we evaluate our method on indoor and outdoor visual localization benchmarks. Specifically, we consider the large-scale \textit{outdoor} Aachen Day-Night v1.1~\cite{Zhang2020AachenV11} and Tokyo24/7~\cite{Torii2015Tokyo247} datasets for localization under severe illumination conditions. Image-based localization in complex \textit{indoor} environments is challenging due to the large viewpoint changes and weakly textured scenes. We use InLoc~\cite{Taira2018InLoc}, a large-scale indoor dataset with strong appearance changes between query images and the reference 3D map. The localization performance on the Aachen Day-Night v1.1 and InLoc benchmarks is reported as the percentage of correctly localized queries. For InLoc, we follow the localization pipeline\footnote{\url{https://github.com/cvg/Hierarchical-Localization}} proposed in~\cite{sarlin2019coarse, sarlin2020superglue}. The query is successfully localized if its camera position and orientation are both within a certain threshold.

The performance on the Tokyo24/7 dataset is evaluated using Recall@N, which is the number of queries that are correctly localized given $N$ nearest neighbor database images. Specifically, for a given query we first obtain a ranked list of database images, $L$ based on Euclidean distance between their global NetVLAD representations. The top-100 ranked database
images, $L^{\prime} \in L$ are re-ranked according to their similarity score based on the number of geometrically verified inliers between the query and each database image.

\customparagraph{Image retrieval.} We evaluate the proposed local image descriptors on the image retrieval benchmark. Specifically, the revisited Oxford ($\cR$Oxford5k) and revisited Paris ($\cR$Paris6k) datasets proposed by Radenovi{\'c}~\etal~\cite{Radenovic2018Revisited} have been used. Similarly to the Tokyo24/7 evaluation protocol, for each query image we first create a ranked list of database images based on cosine similarity of their global representations in the feature space and then compute
2D-2D correspondences between query and top-100 database images which are then re-ranked based on the number of inliers verified by RANSAC. To compute global descriptors, the model "retrievalSfM120k-resnet101-gem" proposed in~\cite{Radenovic2016GEM} is used. We evaluate performance by mean average precision (mAP) and mean precision at 1, 5, and 10 (mP@k), as defined by the protocol~\cite{Radenovic2018Revisited}.

\input{assets/tables/res_retrieval}



\subsection{Results}\label{ssec:results}
First, we experimentally compare the proposed models with their supervised oracles~\cite{Revaud2019R2D2,Wang2020CAPS} on the \textbf{sparse feature matching} benchmark by calculating MMA for different pixel thresholds illustrated in Figure~\ref{fig:hpatches_performance}. Following D2-Net~\cite{Dusmanu2019D2Net}, we separately report results for scenes corresponding to illumination changes (Illumination), viewpoint changes (Viewpoint), and for the whole dataset (Overall). The proposed unsupervised version of R2D2 (R2D2-U) shows a clear improvement over its supervised counterpart (R2D2-S) achieving better results for all evaluation thresholds. At the same time, although CAPS-U demonstrates competitive overall performance, it falls slightly behind its supervised baseline (CAPS-S~\cite{Wang2020CAPS}) on the illumination benchmark at larger pixel thresholds ($>$3px). Our hypothesis is that the original CAPS~\cite{Wang2020CAPS} model that leverages coarse-to-fine architecture (\cf Sec.~\ref{ssec:benchmarks_metrics}) allows to learn more discriminative descriptors leading to better matching performance. We also report homography estimation accuracy, precision (the percentage of correct matches over all the predicted matches) and recall (the ratio of correct matches over the total number of ground truth correspondences) using the same HPatches dataset. Following~\cite{Pautrat2020LISRD}, we use mutual nearest neighbor matcher and a threshold of 3 pixels to consider a match to be correct. The results are summarized in Table~\ref{tbl:hpatches_eval}. As can be seen, the proposed unsupervised models demonstrate competitive performance. Interestingly, the model utilizing global image descriptor for hard-negative mining (CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}-gd) achieves the best Recall and Precision performance over all other methods.

\customparagraph{Visual localization.} We evaluate the performance of the proposed pipeline on the task of image-based localization. Note, that we train our approaches only on outdoor datasets,~\ie Megadepth and Phototourism but evaluate on both outdoor (Aachen v1.1) and indoor (InLoc) to test the generalization of the proposed models. We use R2D2, CAPS and R2D2* as baseline models where R2D2* represents R2D2 model trained with SuperPoint detector, \ie, the setup which is closer to our pipeline (see Sec.~\ref{sec:method}).  For unsupervised methods, we report results obtained by the models utilize in-batch hard-negative sampling during training. The percentage of correctly localized query images is presented in Table~\ref{tbl:loc_aachen_inloc}. First, if we compare R2D2-{$\left(\squarehvfill\right)$} and R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} trained on Aachen database images (A), we can notice that using only synthetic color augmentation is not sufficient to handle drastic illumination changes. Increasing the number of training samples leads to better localization performance. The model R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} trained on (M+P) is comparable to the supervised counterpart on day-time and surpasses it on night-time queries by a noticeable margin: up to $+\textbf{0.5}$ for $\left(0.5m, 5^\circ\right)$ and $+\textbf{1.1}$ for $\left(5m, 10^\circ\right)$. For indoor pose estimation, the same model can outperform the supervised baseline in all metrics: up to $+\textbf{1.5}$ and $+\textbf{2.9}$ for the finest threshold $\left(0.25m, 2^\circ\right)$ for scene DUC1 and DUC2 respectively. Leveraging visual descriptors (*-gd and *-selfgd) provides better outdoor localization results over the models trained with only stylization and color augmentations (R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} and CAPS-{$\left(\squarehvfill,\squarerightblack\right)$}). However, in indoors, visual descriptors \textit{cannot} provide strong generalization performance leading to a marginal improvement (for the R2D2 backbone) or even poor results (with the CAPS backbone). We hypothesize that such behaviour is caused by larger gap in data distribution during training and evaluation. Interestingly, the transferring accuracy depends on the Descriptor CNN (\cf Figure~\ref{fig:pipeline_overview}) structure. The unsupervised model trained on (M+P) and based on the CAPS backbone \textit{cannot} improve performance of outdoor localization compared to its supervised baseline (CAPS~\cite{Wang2020CAPS}). However, large gains are seen for indoor setting: up to $+\textbf{6.1}$ (34.4 \textit{vs.} 40.5) for the most rigorous threshold of scene DUC2. Table~\ref{tbl:loc_tokyo247} shows the localization performance on Tokyo24/7. Similarly to the results on Aachen, R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} is \textit{better} than its supervised counterpart (R2D2-[A+R]) in all metrics: $+\textbf{1.58}$, $+\textbf{1.9}$, and  $+\textbf{1.9}$, respectively. Qualitative results of the proposed models on test images of MegaDepth are illustrated in Figure~\ref{fig:qualitative_results}.


\customparagraph{Image retrieval.} As shown in Table~\ref{tbl:image_retrieval_results}, the proposed unsupervised models show competitive image retrieval performance and surpass their supervised counterparts in mP@k and mAP on $\cR$Oxford5k and $\cR$Paris6k. Most notably, utilizing visual image descriptors with the model based on CAPS backbone leads to better retrieval accuracy which is consistent with the results obtained for the camera localizaton benchmark. However, for the R2D2 backbone model, mining harder negative samples with the help of visual descriptors leads to a marginal improvement (R2D2-{$\left(\squarehvfill,\squarerightblack\right)$} \textit{vs.} R2D2-{$\left(\squarehvfill,\squarerightblack\right)$}-gd) which can be explained by the network capacity. In $\cR$Paris6k both the supervised and unsupervised methods attain comparable performance. Notably, the biggest performance improvement of 5\% is observed across mP@10 under Hard setting.

We observe that increasing the size of dataset ($A \rightarrow M \rightarrow M+P$) performs favourably on the different benchmarks. Stylization provides substantial improvements on Aachen Night time dataset, while performs comparably on other benchmarks. This indicates that the proposed network is not biased to the chosen styles. Furthermore, the proposed coarse-to-fine method with global descriptors also performs favourably compared to in-batch sampling especially on Aachen and $\cR$Oxford5k datasets. Finally, the self-supervised global mining approach *-selfgd performs comparably to *-gd which utilizes image retrieval models pre-trained on SfM data. Improving the on the fly strategy of mining hard negative local samples conditioned on visual image descriptors is a possible future direction.  %


==> hndesc_3dv2021_arXiv_arXiv/sections/introduction.tex <==
\input{assets/images/fig_pipeline}

\vspace{-15pt}
\section{Introduction}~\label{sec:introduction}
Many geometric computer vision tasks require robust estimation of local descriptors such as image alignment~\cite{Balntas2017HPatches}, structure-from-motion~\cite{heinly2015_reconstructing_the_world,schoenberger2016sfm}, image retrieval~\cite{Gordo2017Retrieval,Radenovic2018TPAMI}. With the advent of deep learning models, robust local descriptors can be learnt with highly over-parameterized networks such as Convolutional Neural Networks (CNN). Consequently, much of the latest works~\cite{Balntas2016Localdesc,Detone18superpoint,Dusmanu2019D2Net,Mishchuk2017HardNet,Revaud2019R2D2} have since focused on designing appropriate datasets, labels and loss functions to learn useful local representations.

It is well-known that CNNs are data demanding models that require large amount of data with labelled supervision. While in many cases large amount of data can be obtained, structuring it in meaningful partitions or labels is a costly process. To counter this problem, existing approaches~\cite{Gordo2017Retrieval,Radenovic2016GEM} use SfM pipelines to generate labels. Despite the effectiveness, the process incurs significant computational burden. Furthermore, integrating new stream of data to the existing dataset requires additional iterations of the costly spatial descriptor matching process. The paradigm of self-supervised learning attempts to provide a solution by enabling label-free training of CNNs. Most self-supervised methods focus on auxiliary pretext tasks~\cite{doersch_2015,noroozi_2016,zhang_2016} such as image reconstruction -- generative modelling, or discriminative optimization of the latent space based on contrastive learning~\cite{bachman_2019,dosovitskiy_2014}. The key requirement is to learn transferable representations that can adapt to downstream tasks with limited supervision. Recent progress~\cite{chen2020SimCLR,debiased,he2020moco,kalantidis,robinson_2021} in the image classification domain shows the crucial role of positives (similar) and negatives (dissimilar) in the contrastive loss function to learn robust representations. In this paper, we delve deeper into these factors for the task of local image descriptors learning.

Existing self-supervised methods for learning local descriptors~\cite{Christiansen2019Unsuperpoint,Detone18superpoint} have achieved some success by mining positives and negatives from homography related image pairs (in-pair sampling). On the other hand, \textit{supervised} local descriptor learning methods such as HardNet~\cite{Mishchuk2017HardNet} show consistent improvement with in-batch negative sampling. In addition, image retrieval methods~\cite{Gordo2017Retrieval,Radenovic2016GEM} have demonstrated remarkable results by mining global negative descriptors from a large database of thousands of images. In this paper, we propose a scalable method for sampling hard-negative local features from a wide search space that operates in a coarse-to-fine fashion by leveraging %
image descriptors.

Learning keypoint descriptors that are invariant to illumination changes is a challenging task since it is not easy to acquire suitable data. Synthetic color augmentation (CA) which is widely used to improve model robustness and performance in many computer vision applications~\cite{Fang2019InstaBoost,krizhevsky2012Imagenet,mohan2020efficientps,wu2019detectron2} can enhance illumination invariance of local descriptors only to a certain extent. Following~\cite{Revaud2019R2D2}, we propose to utilize photorealistic image stylization~\cite{Li2018Stylization} at training time. In contrast to~\cite{Revaud2019R2D2}, the more diverse style images are considered which help to increase appearance variations of our training data. We combine these findings to train existing state-of-the-art local descriptor models without any labels. During training and evaluation, only a subset of local descriptors from dense descriptors produced by the network is used. The selection is based on local keypoint detectors such as SuperPoint~\cite{Detone18superpoint} providing efficient training iterations -- by limiting hard-negative mining only to a subset of local descriptors. The proposed method is compared with strong supervised and weakly-supervised baselines~\cite{Revaud2019R2D2,Wang2020CAPS} on a wide range of benchmarks such as visual localization, sparse feature matching, and image retrieval. The key findings are analyzed and complemented by in-depth ablation study.

In summary, this work makes the following contributions: (1) we  demonstrate that improving the quality of hard negative samples during training leads to more powerful and discriminative local keypoint descriptors; (2) by leveraging visual image descriptors, we propose a coarse-to-fine method for mining hard negative local descriptors at scale; (3) we investigate several CA techniques to improve the robustness of learned feature descriptors to illumination changes and show that photorealistic image stylizations yield best performance. We demonstrate that, together, these contributions largely close the gap between self-supervised and fully-supervised approaches for feature descriptor learning. %


==> hndesc_3dv2021_arXiv_arXiv/sections/method.tex <==









\section{Method}\label{sec:method}
In this section, we describe our method for local image descriptors learning that takes a single RGB image and produces a set of local feature descriptors in a self-supervised manner. Supervised methods leverage known scene geometry and utilize image- and keypoint level correspondences to increase robustness and invariance of local features to viewpoint and appearance variations. However, obtaining such ground-truth correspondence might be difficult especially for large-scale scenes. %
We analyze and carefully tailor improvements to existing self-supervised methods for learning invariant local descriptors.

We first review the main components of the proposed approach and the key ideas behind it, then we describe the hard-negative sampling procedure and training loss. An overview of our method is schematically illustrated in Figure~\ref{fig:pipeline_overview}. Given an input image $I_i \in \mathbb{R}^{H\times W\times 3}$ and a set of interest points $\mathbf{k}_i$, our goal is to predict local descriptors $\mathbf{d}_i$ corresponding to index $i$ which would be robust to appearance changes and have good generalization performance. To obtain interest points, we use SuperPoint~\cite{Detone18superpoint} detector. 

\customparagraph{Illumination Invariance}
Illumination invariance can be seen as learning context independent representations. In classification domain, various forms of CA methods such as RandAugment~\cite{Cubuk2019RandAugment} aim to remove the contextual bias in image representations. However, these methods apply various illumination transformations uniformly over both salient foreground object and background context which might be troublesome for local descriptor learning. %
Following~\cite{Melekhov2020Stylization,Revaud2019R2D2} we rely on image stylization~\cite{Li2018Stylization} to improve the robustness of local features under drastic illumination variations. Li~\etal~\cite{Li2018Stylization} propose a closed-form solution to image stylization based on a deep learning model trained in a self-supervised fashion by minimizing the sum of the reconstruction loss and perceptual loss. The method photorealistically transfers style of a reference photo to a content photo preserving local scene geometry. We use this pre-trained model as a part of our pipeline (\textbf{Style CNN} in Figure~\ref{fig:pipeline_overview}) and manually select reference images representing two style categories, \ie night and dusk, from the contributed views of the Amos Patches dataset~\cite{Pultar2019Amos}. In contrast to~\cite{Revaud2019R2D2}, for each category we consider \textit{multiple} style images which are then randomly applied to each image in the training set. The style categories and image stylization results are provided in the supplementary material.

\customparagraph{Viewpoint Invariance.} 
To model viewpoint invariance, recent self-supervised methods~\cite{Christiansen2019Unsuperpoint,Detone18superpoint}
apply a known homography transformation~\textbf{H},~\ie $\hat{I}=\mathbf{H}\left( I \right)$ followed by random crop. As in~\cite{Detone18superpoint}, we use similar types of the homographic adaptation operations: translation, rotation, perspective transform, and scale whose parameters are sampled from a uniform distribution during training (\textbf{H-crops generator}). In addition to stylization, we apply synthetic CA independently on the anchor and positive crops by adding blur, random per-pixel Gaussian noise, adaptive histogram equalization (CLAHE) along with augmentation in brightness, contrast, hue, and saturation. The full list of augmentations is also presented in supplementary.

\customparagraph{Descriptor CNN}. We use a fully-convolutional neural network architecture which takes an input crop $C_i\in \mathbb{R}^{H_c\times W_c\times 3}$ and outputs a dense map of L2-normalized fixed length descriptors, \ie $\mathbb{R}^{H_c\times W_c \times d}$. In this work, we consider two strong baseline methods (supervised and weakly-supervised), namely R2D2~\cite{Revaud2019R2D2} and CAPS~\cite{Wang2020CAPS}. Sec.~\ref{ssec:baselines} provides an overview of these baselines in more detail. In order to perform a fair comparison, we directly use R2D2 and CAPS models as a structure of Descriptor CNN.

\customparagraph{Hard-negative (HN) mining block.}
Supervised metric learning requires both positive and negative samples to learn meaningful representations. Without both positives and negatives, the model will collapse by converging to 0-valued representations. %
Existing unsupervised approaches~\cite{Detone18superpoint,Revaud2019R2D2} for learning local descriptors sample positives and negatives from a homography related image pair $\left(I, \hat{I}\right)$ with local descriptors $A \in I, P \in \hat{I}$ respectively. The images in the pair are dubbed as the anchor ($I$) and to the positive ($\hat{I}$). Each local descriptor $a_i \in A$ is associated with one $p_i \in P$ due to known homography matrix $\mathbf{H}$. Next, for each matching pair $\left(a_i, p_i\right)$ the index $n$ of the non-matching descriptor $p_n$ is obtained as follows:

\begin{equation}
    n = \argmax_{n=1..M, n\neq i} s\left(a_i, p_n\right),
\end{equation}

\noindent where $M$ is the number of interest points in $I$; $s(.)$ is a similarity function such as a dot-product. We refer to this baseline of selecting negatives as in-pair sampling. Several works~\cite{Gordo2017Retrieval,Mishchuk2017HardNet,Radenovic2016GEM} have shown that the quality of negatives has a strong impact in supervised learning of robust representations. Inspired by~\cite{Mishchuk2017HardNet}, we propose in-batch hard negatives sampling strategy that searches non-matching descriptors over all interest point embeddings $p \in B \setminus I$, where $B \sim D$ is a mini-batch sampled from the dataset $D$.

Finding the local hard negatives is an exhaustive process. Sampling negatives over a search space $D_n \sim D$ which is much larger than $B,\quad |D_n|\gg|B|$ ideally should improve the quality of negatives but incurs significant computational cost. Rather than mining hard-negatives at the local descriptor level, we propose a coarse-to-fine search method (\textbf{Image retrieval block} in Figure~\ref{fig:pipeline_overview}). For each image $I \in B$ we first find its nearest neighbor $I^n \in D_n$ in the feature space using visual descriptor $g_n$. This results in a mini-batch $B_n$ consisting of hard-negative image samples (the images look similar to the anchors $I \in B$ but \textit{not} homography related as the positives), \ie, $B_n=\{I_i^n\}_{i=1..|B|}$, which are then used to mine non-matching feature descriptors at the local level. Given the batch, $B_n$ the local descriptor pool now consists of $p_n \in B^\prime \setminus I$ where $B^\prime = (B \cup B_n)$. Such coarse-to-fine strategy leveraging visual image descriptors makes the process of mining hard-negative local descriptors tractable. Computing visual descriptors can be formulated in two ways. On the one hand, one can use state of the art image retrieval models, such as~\cite{Radenovic2016GEM,Radenovic2018TPAMI}, trained on supervised data generated by SfM systems to extract global descriptor from the entire image. On the other hand we propose a completely self-supervised approach whereby the global descriptors are constructed from the set of local descriptors extracted using the current network state. These local descriptors are then aggregated by some mean operation, such as GeM~\cite{Radenovic2016GEM}. %
Specifically, given a dense feature map $X_f \in \mathbb{R}^{H_c\times W_c \times N_d}$, visual descriptor $g_f \in \mathbb{R}^{N_d}$ is obtained by summing \textit{l2} normalized $X_f$ over the spatial resolution. The final representation is again \textit{l2} normalized.




\customparagraph{Loss functions.} Similar to~\cite{He2018LocDesc,Revaud2019R2D2}, we formulate our problem as the optimization of a differentiable approximation ($AP^\prime$) of the Average Precision (AP) ranking metric at training time:

\begin{equation}\label{eq:ap_loss}
    \mathcal{L}_{AP} = \frac{1}{N_a}\sum_i\left(1 - AP^\prime\left(a_i, p_i, \{p_{n_k}^i\}_{k=1..K}\right) \right)
\end{equation}
\noindent where $N_a$ is the number of anchor descriptors in a mini-batch $B^\prime$. In contrast to image matching~\cite{He2018LocDesc}, the number of positive and negative samples is highly imbalanced in our setting. Indeed, for each anchor descriptor in $B^\prime$ there is only one positive sample and several hundred negatives. To address this issue, we propose to select $top$-$K$ hard-negative local descriptors $\{p_{n_k}^i\}_{k=1..K}$ for $a_i$. Results presented in Sec.~\ref{ssec:results} demonstrate consistent improvement over the original AP loss~\cite{He2018LocDesc,Revaud2019R2D2}. For Triplet loss, the proposed idea of intra-batch hard-hegative mining also demonstrates better performance compared to in-pair sampling (see supplementary for more details).




==> hndesc_3dv2021_arXiv_arXiv/sections/related_work.tex <==
\vspace{-10pt}
\section{Related work}~\label{sef:related_work}
\customparagraph{Local image descriptors.} Due to their generalization ability, traditional local features~\cite{Bay2006SURF,Calonder2010BRIEF,Lowe2004SIFT,Rublee2011ORB} are still popular and widely used by many existing systems where establishing pixel correspondences is essential~\cite{Labbe2019RTAB-Map,Mur2017ORB2,schoenberger2016sfm,schoenberger2016mvs}. The recent success of deep learning in various computer vision applications has motivated researchers to work on learned CNN-based approaches for interest point detection~\cite{Barroso2019KeyNet,Lenc2019Detector,Mishkin2018AffNet,Savinov2017detector,Verdie2015TILDE,zhang2017detector}, description~\cite{Balntas2016Localdesc,He2018LocDesc,Luo2019Contextdesc,Mishchuk2017HardNet,Tian2007L2Net,Tian2019SOSNET} or both detection and description~\cite{Detone18superpoint,Dusmanu2019D2Net,Germain2020S2DNet,Luo2020ASLFeat,Ono2018LFNet,Revaud2019R2D2,wang2021p2net,Yi2016LIFT}. Although, those approaches have demonstrated improved performance over classical hand-crafted methods on challenging benchmarks such as vision localization and image matching, most of them require ground-truth pixel correspondences between two views~\cite{Dusmanu2019D2Net,Jiang2021COTR,Revaud2019R2D2,Sun2021LoFTR}. Such accurate ground-truth labels are quite tedious to obtain since it requires information about the 3D representation of the scene (\eg 3D reconstruction, dense depth maps or scene flow). To address this issue, recent research directions have shifted towards weakly- and self-supervised methods. These methods rely on the supervision from epipolar geometry~\cite{Wang2020CAPS,Yang2019EPIPOLAR,Heng2019MONET,Zhou2021Patch2Pix}, principles of Reinforcement Learning~\cite{Bhowmik2020ReinforcedPoints,Truong2019GLAMpoints,Tyszkiewicz2020DISK}, relative camera poses~\cite{Bhowmik2020ReinforcedPoints,Wang2020CAPS}, camera intrinsics~\cite{Heng2021GeomPerc}, and rigid synthetic 2D transformations~\cite{Christiansen2019Unsuperpoint,Detone18superpoint,Revaud2019R2D2,tang2020NeuralRejection}. In this work, we show that with careful choices regarding hard-negative mining, color augmentation and photorealistic image stylization, we can achieve superior performance to supervised methods using only synthetic homographies. In principle, the proposed ideas can be also applied to supervised CNN-based approaches.

\customparagraph{Illumination invariance in feature descriptors.} Learning features that are invariant to illumination changes is a challenging task. To increase robustness to illumination changes, methods like~\cite{Dusmanu2019D2Net,Wang2020CAPS,Heng2021GeomPerc,Yang2020UR2KID} utilize a large SfM database of images with different lighting conditions. Domain adaptation-based methods~\cite{Anoosheh2020S2Night2Day,Mueller2019Image2Image,Porav2018Gans} utilize GANs~\cite{Goodfellow2014GANs,Zhu2017CycleGAN}, view synthesis~\cite{Mueller2019Image2Image} and few-shot learning~\cite{Baik2020DomainAdaptation} to reduce the domain gap between the training and the test (target) image distributions. Leveraging photorealistic image stylization to improve robustness to day-night variations was introduced in~\cite{Revaud2019R2D2}. In the follow-up work, Melekhov~\etal~\cite{Melekhov2020Stylization} extend the original method~\cite{Revaud2019R2D2} by considering more diverse style categories. Pautrat~\etal~\cite{Pautrat2020LISRD} propose a model predicting several dense descriptors with different levels of invariance. For a particular input image, the most relevant invariance is automatically selected using the concept of meta-descriptors based on a NetVLAD~\cite{Arandjelovic2016NetVLAD} layer. Inspired by~\cite{Melekhov2020Stylization,Revaud2019R2D2}, we utilize the idea of image stylization to improve the robustness of local descriptors to appearance variations.

\customparagraph{Self-supervised learning.} Self-supervised learning paves the way for training models on large amount of unlabelled data. Recent methods~\cite{chen2020SimCLR,he2020moco} in the classification domain are based on contrastive loss where representations from augmented copies of the original image -- positives, are contrasted against representations from other images in the batch or memory bank -- negatives. The quality of negatives was analyzed by several methods~\cite{debiased,kalantidis,robinson_2021} in improving self-supervised image representation learning. For local descriptors,~\cite{Laskar2020DensePixelMatching,dgcnet,rocco_17} consider only the augmented input image pair to sample positive and negative local descriptors (in-pair sampling). In this work, we propose methods to improve the quality of both positives and negatives. %


==> introduction.tex <==
\input{assets/images/fig_pipeline}

\vspace{-15pt}
\section{Introduction}~\label{sec:introduction}
Many geometric computer vision tasks require robust estimation of local descriptors such as image alignment~\cite{Balntas2017HPatches}, structure-from-motion~\cite{heinly2015_reconstructing_the_world,schoenberger2016sfm}, image retrieval~\cite{Gordo2017Retrieval,Radenovic2018TPAMI}. With the advent of deep learning models, robust local descriptors can be learnt with highly over-parameterized networks such as Convolutional Neural Networks (CNN). Consequently, much of the latest works~\cite{Balntas2016Localdesc,Detone18superpoint,Dusmanu2019D2Net,Mishchuk2017HardNet,Revaud2019R2D2} have since focused on designing appropriate datasets, labels and loss functions to learn useful local representations.

It is well-known that CNNs are data demanding models that require large amount of data with labelled supervision. While in many cases large amount of data can be obtained, structuring it in meaningful partitions or labels is a costly process. To counter this problem, existing approaches~\cite{Gordo2017Retrieval,Radenovic2016GEM} use SfM pipelines to generate labels. Despite the effectiveness, the process incurs significant computational burden. Furthermore, integrating new stream of data to the existing dataset requires additional iterations of the costly spatial descriptor matching process. The paradigm of self-supervised learning attempts to provide a solution by enabling label-free training of CNNs. Most self-supervised methods focus on auxiliary pretext tasks~\cite{doersch_2015,noroozi_2016,zhang_2016} such as image reconstruction -- generative modelling, or discriminative optimization of the latent space based on contrastive learning~\cite{bachman_2019,dosovitskiy_2014}. The key requirement is to learn transferable representations that can adapt to downstream tasks with limited supervision. Recent progress~\cite{chen2020SimCLR,debiased,he2020moco,kalantidis,robinson_2021} in the image classification domain shows the crucial role of positives (similar) and negatives (dissimilar) in the contrastive loss function to learn robust representations. In this paper, we delve deeper into these factors for the task of local image descriptors learning.

Existing self-supervised methods for learning local descriptors~\cite{Christiansen2019Unsuperpoint,Detone18superpoint} have achieved some success by mining positives and negatives from homography related image pairs (in-pair sampling). On the other hand, \textit{supervised} local descriptor learning methods such as HardNet~\cite{Mishchuk2017HardNet} show consistent improvement with in-batch negative sampling. In addition, image retrieval methods~\cite{Gordo2017Retrieval,Radenovic2016GEM} have demonstrated remarkable results by mining global negative descriptors from a large database of thousands of images. In this paper, we propose a scalable method for sampling hard-negative local features from a wide search space that operates in a coarse-to-fine fashion by leveraging %
image descriptors.

Learning keypoint descriptors that are invariant to illumination changes is a challenging task since it is not easy to acquire suitable data. Synthetic color augmentation (CA) which is widely used to improve model robustness and performance in many computer vision applications~\cite{Fang2019InstaBoost,krizhevsky2012Imagenet,mohan2020efficientps,wu2019detectron2} can enhance illumination invariance of local descriptors only to a certain extent. Following~\cite{Revaud2019R2D2}, we propose to utilize photorealistic image stylization~\cite{Li2018Stylization} at training time. In contrast to~\cite{Revaud2019R2D2}, the more diverse style images are considered which help to increase appearance variations of our training data. We combine these findings to train existing state-of-the-art local descriptor models without any labels. During training and evaluation, only a subset of local descriptors from dense descriptors produced by the network is used. The selection is based on local keypoint detectors such as SuperPoint~\cite{Detone18superpoint} providing efficient training iterations -- by limiting hard-negative mining only to a subset of local descriptors. The proposed method is compared with strong supervised and weakly-supervised baselines~\cite{Revaud2019R2D2,Wang2020CAPS} on a wide range of benchmarks such as visual localization, sparse feature matching, and image retrieval. The key findings are analyzed and complemented by in-depth ablation study.

In summary, this work makes the following contributions: (1) we  demonstrate that improving the quality of hard negative samples during training leads to more powerful and discriminative local keypoint descriptors; (2) by leveraging visual image descriptors, we propose a coarse-to-fine method for mining hard negative local descriptors at scale; (3) we investigate several CA techniques to improve the robustness of learned feature descriptors to illumination changes and show that photorealistic image stylizations yield best performance. We demonstrate that, together, these contributions largely close the gap between self-supervised and fully-supervised approaches for feature descriptor learning. %


==> related_work.tex <==
\vspace{-10pt}
\section{Related work}~\label{sef:related_work}
%\hspace{-3mm}
\customparagraph{Local image descriptors.} Due to their generalization ability, traditional local features~\cite{Bay2006SURF,Calonder2010BRIEF,Lowe2004SIFT,Rublee2011ORB} are still popular and widely used by many existing systems where establishing pixel correspondences is essential~\cite{Labbe2019RTAB-Map,Mur2017ORB2,schoenberger2016sfm,schoenberger2016mvs}. The recent success of deep learning in various computer vision applications has motivated researchers to work on learned CNN-based approaches for interest point detection~\cite{Barroso2019KeyNet,Lenc2019Detector,Mishkin2018AffNet,Savinov2017detector,Verdie2015TILDE,zhang2017detector}, description~\cite{Balntas2016Localdesc,He2018LocDesc,Luo2019Contextdesc,Mishchuk2017HardNet,Tian2007L2Net,Tian2019SOSNET} or both detection and description~\cite{Detone18superpoint,Dusmanu2019D2Net,Germain2020S2DNet,Luo2020ASLFeat,Ono2018LFNet,Revaud2019R2D2,wang2021p2net,Yi2016LIFT}. Although, those approaches have demonstrated improved performance over classical hand-crafted methods on challenging benchmarks such as vision localization and image matching, most of them require ground-truth pixel correspondences between two views~\cite{Dusmanu2019D2Net,Jiang2021COTR,Revaud2019R2D2,Sun2021LoFTR}. Such accurate ground-truth labels are quite tedious to obtain since it requires information about the 3D representation of the scene (\eg 3D reconstruction, dense depth maps or scene flow). To address this issue, recent research directions have shifted towards weakly- and self-supervised methods. These methods rely on the supervision from epipolar geometry~\cite{Wang2020CAPS,Yang2019EPIPOLAR,Heng2019MONET,Zhou2021Patch2Pix}, principles of Reinforcement Learning~\cite{Bhowmik2020ReinforcedPoints,Truong2019GLAMpoints,Tyszkiewicz2020DISK}, relative camera poses~\cite{Bhowmik2020ReinforcedPoints,Wang2020CAPS}, camera intrinsics~\cite{Heng2021GeomPerc}, and rigid synthetic 2D transformations~\cite{Christiansen2019Unsuperpoint,Detone18superpoint,Revaud2019R2D2,tang2020NeuralRejection}. In this work, we show that with careful choices regarding hard-negative mining, color augmentation and photorealistic image stylization, we can achieve superior performance to supervised methods using only synthetic homographies. In principle, the proposed ideas can be also applied to supervised CNN-based approaches.

\customparagraph{Illumination invariance in feature descriptors.} Learning features that are invariant to illumination changes is a challenging task. To increase robustness to illumination changes, methods like~\cite{Dusmanu2019D2Net,Wang2020CAPS,Heng2021GeomPerc,Yang2020UR2KID} utilize a large SfM database of images with different lighting conditions. Domain adaptation-based methods~\cite{Anoosheh2020S2Night2Day,Mueller2019Image2Image,Porav2018Gans} utilize GANs~\cite{Goodfellow2014GANs,Zhu2017CycleGAN}, view synthesis~\cite{Mueller2019Image2Image} and few-shot learning~\cite{Baik2020DomainAdaptation} to reduce the domain gap between the training and the test (target) image distributions. Leveraging photorealistic image stylization to improve robustness to day-night variations was introduced in~\cite{Revaud2019R2D2}. In the follow-up work, Melekhov~\etal~\cite{Melekhov2020Stylization} extend the original method~\cite{Revaud2019R2D2} by considering more diverse style categories. Pautrat~\etal~\cite{Pautrat2020LISRD} propose a model predicting several dense descriptors with different levels of invariance. For a particular input image, the most relevant invariance is automatically selected using the concept of meta-descriptors based on a NetVLAD~\cite{Arandjelovic2016NetVLAD} layer. Inspired by~\cite{Melekhov2020Stylization,Revaud2019R2D2}, we utilize the idea of image stylization to improve the robustness of local descriptors to appearance variations.

\customparagraph{Self-supervised learning.} Self-supervised learning paves the way for training models on large amount of unlabelled data. Recent methods~\cite{chen2020SimCLR,he2020moco} in the classification domain are based on contrastive loss where representations from augmented copies of the original image -- positives, are contrasted against representations from other images in the batch or memory bank -- negatives. The quality of negatives was analyzed by several methods~\cite{debiased,kalantidis,robinson_2021} in improving self-supervised image representation learning. For local descriptors,~\cite{Laskar2020DensePixelMatching,dgcnet,rocco_17} consider only the augmented input image pair to sample positive and negative local descriptors (in-pair sampling). In this work, we propose methods to improve the quality of both positives and negatives. %

